Scheduling Precedence-Constrained Jobs on Related Machines with Communication Delay

We consider the problem of scheduling $n$ precedence-constrained jobs on $m$ uniformly-related machines in the presence of an arbitrary, fixed communication delay $\rho$. We consider a model that allows job duplication, i.e. processing of the same job on multiple machines, which, as we show, can reduce the length of a schedule (i.e., its makespan) by a logarithmic factor. Our main result is an $O(\log m \log \rho / \log \log \rho)$-approximation algorithm for minimizing makespan, assuming the minimum makespan is at least $\rho$. Our algorithm is based on rounding a linear programming relaxation for the problem, which includes carefully designed constraints capturing the interaction among communication delay, precedence requirements, varying speeds, and job duplication. Our result builds on two previous lines of work, one with communication delay but identical machines (Lepere, Rapine 2002) and the other with uniformly-related machines but no communication delay (Chudak, Shmoys 1999). We next show that the integrality gap of our mathematical program is $\Omega(\sqrt{\log \rho})$. Our gap construction employs expander graphs and exploits a property of robust expansion and its generalization to paths of longer length. Finally, we quantify the advantage of duplication in scheduling with communication delay. We show that the best schedule without duplication can have makespan $\Omega(\rho/\log \rho)$ or $\Omega(\log m/\log\log m)$ or $\Omega(\log n/\log \log n)$ times that of an optimal schedule allowing duplication. Nevertheless, we present a polynomial time algorithm to transform any schedule to a schedule without duplication at the cost of a $O(\log^2 n \log m)$ factor increase in makespan. Together with our makespan approximation algorithm for schedules allowing duplication, this also yields a polylogarithmic-approximation algorithm for the setting where duplication is not allowed.

==> MkU_Upper_Bound.tex <==
\section{Upper bound from MkU }

We can get an upper bound from the algorithm for the Minimum $k$-Union  problem ($\mku$) given in \cite{chlamtavc2017minimizing}, by using it as a black box. 

\begin{definition}{Minimum $k$-Union problem ($\mku$).}
We are given a universe $U$ of $n$ elements, a collection of $m$ subsets: $\mathcal{S} \subseteq \cP(U)$, and an integer $k \leq m$. The objective is to return a collection of subsets $\mathcal{T} \subseteq \mathcal{S}$ of size $k$ that minimizes the size of their union, i.e. minimize $|\cup_{T \in \mathcal{T}} T|$ subject to $|\mathcal{T}| = k$.
\end{definition}

Suppose we can solve the $\mku$ problem exactly, the question we are trying to answer here is, whether it gives us any upper bound for the approximation factor for the DAG scheduling problem, that we can obtain using the solution to the related $\mku$ problem. We answer this question with $\log n$. Then, we qualify our statement saying that since the best approximation given for $\mku$ is $O(l^{1/4 +\e})$, it gives us an  $O(l^{1/4 + \e} \log l)$-approximation algorithm, and hence the upper bound. \zoya{What's $l$?}
We consider the case where there are $l$ leaves in the DAG \zoya{rename leaves to sinks} and there are $m$ machines, and the communication delay $\rho$ is large. In such a case, in an optimal schedule, no machine communicates with another. Therefore, the set of jobs is partitioned according to the predecessor sets of the leaves and each machine is allocated a set of such sets. An upper bound for this case will be an upper bound in general, as communication can only increase the makespan.


\begin{lemma}
For large $\rho$, the DAG scheduling problem has an $O(n^{1/4 + \e} \log n )$-approximation algorithm. \zoya{I think this needs to say what ``large'' means for it to be a lemma}
\end{lemma}

\begin{proof}

Let $L$ be the set of leaves in the DAG G. For each leaf $i \in L$, let $S_i$ denote the set of predecessors of $i$. The size of this collection be denoted by $l:= |L|$.
We aim to partition the sets $S_i$ into $m$ sets, viz. $\inbr{P_1, P_2, P_m}$ such that the set of jobs placed in machine $i$ is denoted by \[\bigcup_{S \in P_i} S\]
 
 Denote the set of all possible partitions of the nodes of $G$ by $\cP(G)$. We denote by $M^*$ the optimum obtained as follows:
 
 \[M^* = \min_{ \inpa{P_i}_{i=1}^m \in \cP(G)} \max_i |\bigcup_{S \in P_i} S|\]

We use the oracle $\O_{MkU}$ for the MkU instances to obtain this optimum.

\begin{algorithm}[H]
\KwData{DAG $G$}
\KwResult{Schedule with $\log \ell$ approximation}
$j \leftarrow 1$\;
\While{there is some $S_i$ yet to be scheduled}{
    $k \leftarrow \ell / (m 2^j)$\;
    $\{ T_1, T_2, \ldots, T_k \} \leftarrow \mathcal{O}_{MkU}\big[k, %\frac{\ell}{m2^j}, 
    \mathcal{S} \big]$, that covers $1/2^j$ sets \zoya{which sets?} \;
    schedule these sets on arbitrary $k$ machines \zoya{there may not be $k$ machines} with residual capacity \zoya{what's residual capacity?} \;
    $j \leftarrow j+1$\;
}
\caption{Constructs a schedule for large $\rho$}
\end{algorithm}

% ------- old version ------%
\iffalse
\begin{algorithm}
    \caption{on input: DAG $G$ \newline
    output: schedule with $\log \ell$ approximation}
\begin{algorithmic}[1]
    \STATE $j = 1$
    \WHILE{there is some $S_i$ yet to be scheduled}
        \STATE $k \leftarrow \frac{\ell}{m2^j}$
        \STATE $\inbr{T_1, T_2, \cdots T_k} \leftarrow\O_{MkU}\insq{\frac{\ell}{m2^j}, \mathcal{S}}$, that covers $\frac{1}{2^j}$ sets 
        \STATE schedule these sets on arbitrary $k$ machines with residual capacity
        \STATE $j \leftarrow j+1$
    \ENDWHILE    
\end{algorithmic}    
\end{algorithm}
\fi
%------- end old version ------%

[This while loop can continue for $j \leq \log l$ iterations at most. At each iteration it finds an optimal schedule for $l/2^j$ sets.]

If there are $c$ such iterations after which no set is left uncovered, we stop. Certainly, $c \leq \log l$.

Since we can replace the oracle $\O(\mku)$ with the polynomial time algorithm guaranteed in theorem 1.6 of \cite{chlamtavc2017minimizing} to solve any instance of $\mku$ with an approximation factor of $O(l^{1/4 +\e})$, together with the algorithm above, the approximation factor will be $O(l^{1/4 +\e} \log l)$.

\textbf{In progress.}
Now, we analyze the approximation factor obtained by this greedy algorithm together with the approximation algorithm for $\mku$, compared to the optimal algorithm for the DAG scheduling problem, $\opt$.

% \begin{align*}
% f(U_s) &\leq (1-e^{r/s})(l^{1/4 + \e}\log l) \opt\\
% \end{align*}

Suppose $\opt_j$ is the optimal cover for iteration $j$, and there are $L_j$ elements left to cover. By pigeonhole principle, there is a collection of sets that cover $L_j/\opt_j$. Therefore, the greedy choice obtained is at least as good. Therefore, 
% $L_j \leq L_{j-1} - \frac{L_{j-1}}{\opt_{j-1}} \leq \leq L_{j-1} - \frac{L_{j-1}}{\opt}$

\begin{align*}
    L_j &\leq L_{j-1} - \frac{L_{j-1}}{\opt_{j-1}}\\
    &\leq L_{j-1} - \frac{L_{j-1}}{\opt}\\
    &= \inpa{1-\frac{1}{\opt}}L_{j-1}\\
\end{align*}

Therefore, after $k$ iterations,

\begin{align*}
    L_0 &\leq (1-\frac{1}{\opt})L_{1}\\
    &\leq \inpa{1- \frac{1}{\opt}}^k L_k\\
\end{align*}



\end{proof}

==> MoreMotivation/PhaseVariableLP.tex <==
\newcommand{\phaseLP}{(\ref{phaseLP_delay}-\ref{phaseLP_samephase})}

Unit speeds and job sizes:

\begin{align}
    \start{v} &\ge \start{u} + \delay(1-\phasevariable{u}{v}) &\forall u \prec v
    \\
    \sum_{u \in \predex{v}} \proc{v} \phasevariable{u}{v} &\le \delay   &\forall v
    \\
    \start{v} &\ge \start{u} + 1 &\forall u \prec v
    \\
    \LPmakespan &\ge \start{v} + 1 &\forall v
    \\
    \LPmakespan &\ge \sum_v \jobmachine{v}{i} &\forall i
    \\
    \sum_i  \jobmachine{v}{i} &= 1 &\forall v
    \\
    \start{v} &\ge 0 &\forall v
    \\
    \jobmachine{v}{i} &\in (0,1) &\forall v,i
    \\
    \phasevariable{u}{v} &\in (0,1) &\forall u,v
\end{align}

First attempt at non-unit speeds and job sizes:

\begin{align}
    %\phasevariable{u}{u'} &\le \phasevariable{u}{v} &\forall u \prec u', u' \prec v 
    %\\
    %\phasevariable{u}{v} &\le \phasevariable{u'}{v} &\forall u \prec v, u' \prec v, u \prec u'
    %\\
    \start{v} &\ge \start{u} + \delay(1-\phasevariable{u}{v}) &\forall u \prec v
    \\
    \sum_{u \in \predex{v}} \proc{u} \phasevariable{u}{v} &\le \delay \sum_{i}  \speed{i} \jobmachine{v}{i}  &\forall v
    \\
    \start{v} &\ge \start{u} + \proc{u} \sum_i  \jobmachine{u}{i} / \speed{i} &\forall u \prec v
    \\
    \LPmakespan &\ge \start{v} + \proc{v} \sum_i \jobmachine{v}{i} / \speed{i} &\forall v
    \\
    \LPmakespan\speed{i} &\ge \sum_v \proc{v} \jobmachine{v}{i} &\forall i
    \\
    \sum_i  \jobmachine{v}{i} &= 1 &\forall v
    \\
    \start{v} &\ge 0 &\forall v
    \\
    \jobmachine{v}{i} &\in (0,1) &\forall v,i
    \\
    \phasevariable{u}{v} &\in (0,1) &\forall u,v
\end{align}

Second attempt at non-unit speeds and job sizes:

\begin{align}
    \delay \speed{i} \sum_{j \le i} \jobmachine{v}{j} &\ge \sum_{u \in \predex{v}} \proc{u} \machinephase{u}{v}{i}    &\forall v, i
    %\label{phaseLP_phasepredecessors}
    \\
    \start{v} &\ge \start{u} + \delay \Big( \sum_{j \le i} \jobmachine{v}{j} - \machinephase{u}{v}{i} \Big) &\forall u \prec v, i
    %\label{phaseLP_delay}
    \\
    \start{v} &\ge \start{u} + \proc{u} \sum_i  \jobmachine{u}{i} / \speed{i} &\forall u \prec v
    %\label{phaseLP_execution}
    \\
    \LPmakespan &\ge \start{v} + \proc{v} \sum_i \jobmachine{v}{i} / \speed{i} &\forall v
    %\label{phaseLP_completionlb}
    \\
    \LPmakespan\speed{i} &\ge \sum_v \proc{v} \jobmachine{v}{i} &\forall i
    %\label{phaseLP_loadlb}
    \\
    \sum_i  \jobmachine{v}{i} &= 1 &\forall v
    %\label{phaseLP_finishjob}
    \\
    \start{v} &\ge 0 &\forall v
    %\label{phaseLP_nonnegstart}
    \\
    \jobmachine{v}{i} &\in (0,1) &\forall v,i
    %\label{phaseLP_jobmachine}
    \\
    \machinephase{u}{v}{i} &\in (0,1) &\forall u,v,i
    %\label{phaseLP_samephase}
\end{align}

To understand the linear program, think of any schedule as being divided into \textit{phases} of time of length $\delay$. We can see that within a phase there is no communication between any machines. So if a job and any of its predecessors are scheduled to start in the same phase then they must be scheduled on the same machine. Therefore, if a job is executed on a machine of speed $s$ then the total number of its predecessors that are scheduled in the same phase is at most $\delay s$.
%Intuitively, then, we can think of $\machinephase{u}{v}{i}$ as indicating whether or not to schedule $u$ and $v$ in the same phase, given that $v$ is scheduled on a machine of speed (at least) $\speed{i}$. 

Intuitively, then, we can think of the values of $\jobmachine{u}{i}$ as giving the \textit{primary} placement of $u$. That is, if we want to finish $u$ as quickly as possible, we should place it on a machine where it has high mass according to $\jobmachine{u}{i}$. We can then think of $\machinephase{u}{v}{i}$ as giving the \textit{secondary} placement of $u$. That is, if we want to finish $v$ as quickly as possible, we should place $v$ on a machine $j$ where it has a lot of mass according to $\jobmachine{v}{i}$ and, if $\machinephase{u}{v}{j}$ is large, we should make a \textit{copy} of $u$ to execute in the same phase as $v$ on $j$.

Constraint~(\ref{phaseLP_delay}) states the communication delay requirement in terms of start times. Constraint~(\ref{phaseLP_phasepredecessors}) states that the total size of all predecessors that start less $\delay$ time before $v$ is executed on machine $i$ is less than $\delay \speed{i}$.

\begin{lemma}
    \LP{\phaseLP}{} is a valid relaxation of DAG Scheduling with Communication Delay. 
\end{lemma}

\begin{proof}
    Let $\sigma$ be any schedule. We set the variables of \LP{\phaseLP}{} as follows. For each $v$, let $i^*$ be some machine on which $v$ first completes, choosing arbitrarily if there is more than one. Let $t^*$ be the earliest start time of $v$ on $i^*$ and set $\start{v} = t^*$. Set $\jobmachine{v}{i^*} = 1$ and $\jobmachine{v}{i} = 0$ for $i \ne i^*$. Set $\machinephase{u}{v}{i} = 0$ for all $i < i^*$. For $u \prec v$ and $i \ge i^*$, set $\machinephase{u}{v}{i} = 1$ if $\start{v} - \start{u} \le \delay$, and $\machinephase{u}{v}{i} = 0$ otherwise. Set $C$ to the makespan of $\sigma$.
    
    The satisfaction of constraints (\ref{phaseLP_execution}) - (\ref{phaseLP_samephase}) is either trivial or follows from the same reasoning as our old LP. 
    For Constraint~(\ref{phaseLP_delay}) if we fix $u,v$ and $i$ and let $\sum_{j \le i} \jobmachine{v}{j} = \alpha$ and $\machinephase{u}{v}{i} = \beta$, then there are four cases (a) $\alpha =\beta = 1$, (b) $\alpha= 1$ and $\beta = 0$, (c) $\alpha = 0$ and $\beta = 1$, or (d) $\alpha = \beta = 0$. In cases (a), (c), and (d) it is easy to see that the constraint is satisfied by the fact that $\start{v} \ge \start{u}$. In case (b), we see that $\machinephase{u}{v}{i}$ is set to 0 only when $\start{v} - \start{u} \ge \delay$, which entails that constraint is satisfied, or when $i < i^*$, which entails $\sum_{j \le i} \jobmachine{v}{j} = 0$.
    
    To show Constraint~(\ref{phaseLP_phasepredecessors}) is satisfied, fix $v$ and $i$ and let $A$ be the set of jobs $u \in \predex{v}$ for which $\machinephase{u}{v}{i} = 1$. By our setting of $\machinephase{u}{v}{i}$, if $\sum_{j \le i} \jobmachine{v}{i} = 0$, then $A = \varnothing$ and the constraint is trivially satisfied. So assume that $\sum_{j \le i} \jobmachine{v}{i} = 1$. This implies that $v$ is first completed on a machine no faster than $\speed{i}$. All jobs in $A$ start their first completed execution less than $\delay$ time before the start of $v$. So the total size of $A$ is at most $\delay\speed{i}$.
\end{proof} 

\begin{definition}
    Band $\band{r}= \{v: \delay(r-1)/4 \leq \start{v} < \delay r/4\}$. 
\end{definition}

\begin{lemma}
    Let $\LPopt$ be the optimal value of \LP{\phaseLP}{} and let $r^* = \max \{r: \band{r} \ne \varnothing\}$. Then $\delay r^* \le 4(\LPopt+\delay)$.
\end{lemma}

\begin{proof}
    For any job $v \in \band{r^*}$, we have that $\start{v} \ge \delay(r^*-1)/4$ by definition of $\band{r^*}$. So
    $\delay r^* = 4\frac{\delay(r^*-1)}{4} + \delay \le 4\start{v} + \delay \le 4(\LPopt + \delay)$ by Constraint (\ref{phaseLP_completionlb}).
\end{proof}

\begin{definition}
    $\med{v} = \min \{i : \sum_{j \le i} \jobmachine{v}{j} \ge \sfrac{1}{2}\}$.
\end{definition} 

\begin{lemma}
    Let $v$ be any job, $r$ be the band that contains $v$, and $i^* = \med{v}$. Then $\setproc{\predex{v} \cap \band{r}} \le 4\delay \speed{i^*}$.
\end{lemma}

\begin{proof}
    Let $A = \predex{v} \cap \band{r}$. Then, for any $u \in A$,
    \begin{align*}
        \start{v} &\ge \start{u} + \delay \Big( \sum_{j \le i^*} \jobmachine{v}{j} - \machinephase{u}{v}{i^*} \Big) &\text{by (\ref{phaseLP_delay})}
        \\
        &\ge \start{u} + \delay ( \sfrac{1}{2} - \machinephase{u}{v}{i^*} ) &\text{by definition of } i^*.
    \end{align*}
    Since $\start{v} \le \start{u} + \delay/4$ (by definition of $\band{r}$), we have that $\machinephase{u}{v}{i^*} \ge \sfrac{1}{4}$ for all $u \in A$. 
    Suppose for the sake of contradiction that $\setproc{A} > 4 \delay\speed{i^*}$. Then
    \begin{align*}
        \sum_{u \in \predex{v}} \proc{u} \machinephase{u}{v}{i^*} &\ge \sum_{u \in A} \proc{u} \machinephase{u}{v}{i^*} \ge  \setproc{A}/4 > \delay \speed{i^*} &\text{by assumption}
        \\
        &= \delay \speed{i^*} \sum_j \jobmachine{v}{j} \ge \delay \speed{i^*} \sum_{j \le i^*} \jobmachine{v}{j} &\text{by (\ref{phaseLP_finishjob}).}
        %\\
        %&= 2 \delay  \sum_j \speed{i} \jobmachine{v}{j} \ge 2 \delay \sum_{j \le i} \speed{j} \jobmachine{v}{j} &\text{by the order of machines}
        %\\
        %&\ge 2 \delay (1/2) \sum_j \speed{j} \jobmachine{v}{j} =  \delay \sum_j \speed{j} \jobmachine{v}{j} &\text{by definition of}~ i.
    \end{align*}
    Therefore, Constraint~(\ref{phaseLP_phasepredecessors}) is violated.
\end{proof}

We assign jobs to groups as we did before, so Lemma~\ref{lem:LoadBound} goes through exactly the same way.

\david{The following lemma isn't necessary, but would give further evidence that this new LP can replace the old. Not finished.}

\begin{lemma}
    Take any solution $\vector{x}^* = \{\machinephase{u}{v}{i}\}_{u,v,i} \cup \{ \jobmachine{v}{i}\}_{v,i} \cup \{S_v\}_v$ to \LP{\phaseLP}{}. Let $\vector{x} = \vector{x}^* \cup \{\comp{v}\}_v$ where $\comp{v} = \start{v} + \proc{v} \sum_i \jobmachine{v}{i}/\speed{i}$. Then $\vector{x}$ is a feasible solution to \LP{}{}.
\end{lemma}

\begin{proof}
    We prove that each constraint of \LP{}{} is satisfied by $\vector{x}$. For all $v$,  (\ref{LP:Gen:makespan}) is satisfied by (\ref{phaseLP_completionlb}) and definition of $\comp{v}$. For all $v$, (\ref{LP:Gen:predecessor}) is satisfied by (\ref{phaseLP_execution}) and definition of $\comp{v}$. For all $v$, (\ref{LP:Gen:execution}) is satisfied by definition of $\comp{v}$. (\ref{LP:Gen:load}), (\ref{LP:Gen:cover}), (\ref{LP:Gen:nonneg_start}), and (\ref{LP:Gen:nonneg_indicator}) are satisfied by (\ref{phaseLP_loadlb}), (\ref{phaseLP_finishjob}), (\ref{phaseLP_nonnegstart}), and (\ref{phaseLP_jobmachine}), respectively. So, we just need to show that (\ref{LP:Gen:height}) and (\ref{LP:Gen:large_size_height}) are satisfied.
    
    We show that (\ref{LP:Gen:large_size_height}) is satisfied. Let $v$ be any job and $u$ any job that precedes $v$. Let $i$ be any machine such that $\proc{u} \ge \delay\speed{i}$. 
\end{proof}

==> Old Makespan/analysis.tex <==
Our analysis combines elements of the analysis given in \cite{chudak1999approximation} and \cite{LR02}. As in \cite{chudak1999approximation}, we define a chain of jobs whose execution time serves as a lower bound on the optimal length of any schedule. 
The chain also has the following property: for any non-chain job $v$ that precedes a job in the chain and is not executed in parallel with the chain, $v$'s execution time is no longer than $\delay$. This property allows us to leverage the analysis from \cite{LR02} to show that the time spent in $\sigma$ not executing the chain can be bounded by the highest band number and the load on all groups, both of which give lower bounds on the optimal makespan. 

We define the \textit{chain} $\chain = \{ \link{1}, \link{2} , \ldots, \link{|\chain|} \}$ as follows. Let $D$ be the set of pairs that determine start times in $\sigma$, i.e.\ the pairs $(v,i)$ such that $\sigma[v,i] \ne \bot$. Let $L$ be the set of pairs that determine the start times of long jobs, i.e.\ the set of pairs
$(v,i) \in D$ such that $\proc{v}/\speed{i} > \delay$. Then 
\begin{align*}
    \link{|\chain|} &= \arg\max_{(v,i) \in L} \{ \sigma[v,i] + \proc{v}/\speed{i} \} \quad\quad \text{and, for}~ q < |\chain|,
    \\
    \link{q} &= \arg\max_{(v,i) \in L} \{\sigma[v,i] + \proc{v}/\speed{i} : v \in \predex{u} ~\text{and}~ \sigma[v,i] + \proc{v}/\speed{i} \le \sigma[u,j] + \proc{u}/\speed{j} ~\text{where}~ \link{q+1} = (u,j) \} .
\end{align*}
We also define sets of jobs that precede jobs in the chain and execute between jobs in the chain. 
Let $V_{|\chain|}$ be the set of jobs that complete after $\link{|\chain|}$, i.e. for $\link{|\chain|} = (i,v)$, let $V_{|\chain|}$ be the set of $u \in V$ such that, for some machine $j$ we have $(u,j) \in D$ and $\sigma[u,j] + \proc{u}/\speed{j} \ge \sigma[v,i] + \proc{v}/\speed{i}$.
Then let $V_q$ be the set of predecessors of the next job in the chain that complete after the previous job in the chain (if it exists), i.e.\ for $\link{q+1} = (v,i)$, let $V_{q}$ be the set of all jobs $u$ such that there is some machine $j$ where $(u,j) \in D$ and $u \in \predex{v}$ and $\sigma[u,j] + \proc{u}/\speed{j} \le \sigma[v,i]$ and, if $\link{q-1} = (v',i')$ exists, $\sigma[u,j] + \proc{u}/\speed{j} \ge \sigma[v',i'] + \proc{v'}/\speed{i'}$.
Figure \ref{fig:chain_construction} depicts the construction of $\chain$ and each $V_q$.

\begin{figure}
    \centering
    \includegraphics[scale=.8]{Figures/chain_construction_new.pdf}
    \caption{Machines are shown vertically on the left and time increases from left to right. The dotted lines track the jobs being executed on each machine. Jobs $v_1$ through $v_5$ are the only jobs with copies that take longer than $\delay$ time. Other jobs are scheduled but not shown. In this case, $\chain = \{ \link{1} : (v_1, 2), \link{2}:(v_2, 4), \link{3}:(v_3, 2), \link{4}:(v_4,5), \link{5}:(v_5,3)\}$. The sets $V_q$ are shown as shaded regions. All jobs $v$ such that some copy of $v$ is scheduled on $i$ and the completion time of $v$ on $i$, given by $\sigma[v,i] + \proc{v}/\speed{i}$, falls inside the shaded rectangular region is a member of $V_5$. All jobs $v \in \predex{v_{q+1}}$ such that some copy of $v$ is scheduled on $i$ and the completion time of $v$ on $i$ falls inside the shaded trapezoidal region to the left of $v_{q+1}$ are elements of $V_q$.}
    \label{fig:chain_construction}
\end{figure}

We now upper bound the total processing time spent executing $\chain$ in $\sigma$ in terms of $\guess$. Recall that the group assigment used in Algorithm~\ref{alg:Gen:scheduler} was derived from the solution to \NCP{}{\guess}.

\begin{lemma}[{\bf Lower bound on $\guess$ in terms of the chain}]
    \[\displaystyle \sum_{v \in \chain} \frac{\proc{v}}{\groupspeed{\assign{v}}} \le 4\guess . \]
    \label{lem:ChainBound}
\end{lemma}

\begin{proof}
    Recall that $\chain = \{ \link{1}, \ldots, \link{|\chain|} \}$. We claim that for any $\link{y} \in \chain$ where $\link{y} = (v,i)$ we have that
    \[\comp{v} \ge \sum_{x \le y : \link{x} = (u,j)} \frac{\proc{u}}{4\groupspeed{\assign{u}}}. \]
    By constraint (\ref{LP:Gen:makespan}) and (\ref{LP:guess}), this is sufficient to prove the lemma. 
    
    We prove the claim by induction.
    \junk{For $\link{1}  = (v, i)$, we have that 
    \[ \comp{v} \ge \sum_j \frac{\proc{v}\LPind{v}{j}}{\speed{j}} \ge \frac{\proc{v}}{4 \groupspeed{\assign{v}}}  \]
    by Constraint (\ref{LP:Gen:execution}) and definition of $\assign{v}$.}
    We prove the inductive step first.
    Suppose the claim holds for $\{ \link{1}, \ldots, \link{x} \}$ with $\link{x} = (v',i')$ and $\link{x+1} = (v,i)$. By definition of $\chain$, we have that $u \in \predex{v}$. Then
    \begin{align*}
        \comp{v} &\ge \sum_j \frac{\proc{v} \LPind{v}{j}}{\speed{j}} + \comp{v'} &\text{by Constraints (\ref{LP:Gen:predecessor}) and (\ref{LP:Gen:execution}) }
        \\
        &\ge \sum_{k \le \assign{v}} \sum_{j \in \group{k}} \frac{\proc{v} \LPind{v}{j}}{\speed{j}} + \comp{v'} 
        \\
        &\ge \sum_{k \le \assign{v}} \sum_{j \in \group{k}} \frac{\proc{v} \LPind{v}{j}}{2\groupspeed{\assign{v}}} + \comp{v'} &\text{by definition of}~ \groupspeed{\assign{v}}
        \\
        &\ge \frac{\proc{v}}{4\groupspeed{\assign{v}}} + \comp{v'} &\text{by definition of}~ \assign{v} 
        \\
        &\ge \sum_{y \le x+1: \link{y} = (u,j)} \frac{\proc{u}}{4\groupspeed{\assign{u}}} &\text{by induction.}
    \end{align*}
    The base case follows similarly, without assuming the existence of $v'$. The lemma follows.
\end{proof}

We now prove several results regarding the time spent by $\sigma$ not executing jobs in the chain. For this purpose, we partition the phase indices of $\sigma$ into two sets, $\Phi$ and $\Phi_{\chain}$. We define the set $\Phi$ to be those phase indices $\tau$ where less than $\delay$ time is spent executing jobs in $\chain$. All other phases are elements of $\Phi_{\chain}$.

\begin{lemma}[{\bf Completion time of chain jobs in a phase in $\Phi$}]
    For all $\tau \in \Phi$, if any part of $v \in \chain$ is executed in phase $\tau$ then $v$ must end its execution before time $\phaselength \tau + \delay$.
    \label{lem:non_chain_phase_execution}
\end{lemma}

\begin{proof}
    Suppose some fraction of $v$ were executed at time after $\phaselength\tau + \delay$. Then either $v$ is started in phase $\tau$ or in some previous phase. If it is started in a previous phase, then it must have executed from time $\phaselength\tau$ to $\phaselength\tau + \delay$. If $v$ starts in phase $\tau$, then its starting time is before $\phaselength\tau + 4\delay$. In either case it executes for at least $\delay$ time in the phase, which contradicts $\tau \in \Phi$.
\end{proof}

We also classify the phases according to how much work is done on each group in the phase.
We say that phase $\tau$ is a \textit{load phase of group} $k$ if every machine $j \in \group{k}$ is such that $j$ is processing jobs for at least $\delay$ time in $\tau$. If in phase $\tau$ for every group $k$ there is some machine $j$ such that $j$ is processing jobs for less than $\delay$ time, then we say that $\tau$ is a \textit{height} phase. 

\begin{lemma}
    For any phase $\tau \in \Phi$, if $\tau$ is a height phase then either $\tau$ is the last phase of $\sigma$ or there is some $q$ such that, for some job $v \in V_q$, $v$ is not completed before time $\phaselength\tau$. 
    \label{lem:height_phase_limit}
\end{lemma}

\begin{proof}
    To prove this claim, suppose $\tau$ is a height phase and consider the first iteration $t$ of the outer while-loop in Algorithm \ref{alg:Gen:scheduler} in which the phase index variable $\algofont{\tau}$ has value $\tau$. Suppose, for the sake of contradiction, that $\tau$ is not the last phase of $\sigma$ and, for all $q$, $V_q$ has finished all jobs by the start of phase $\tau$.  By Lemma~\ref{lem:non_chain_phase_execution} and $\tau \in \Phi$, we have that no chain job executes in $\tau$ after time $\phaselength\tau + \delay$. If the chain job $v_{|\chain|}$ completes in or before phase $\tau$ then $\tau$ is the last phase of $\sigma$. So assume that there is some chain job $v_q$ that is not started before phase $\tau$. Since $\tau$ is a height phase, we know that there is some machine $i \in \group{\assign{v_q}}$ that ends its execution of all jobs in $\tau$ before time $\phaselength\tau + \delay$. So, we know that $i$ satisfies (C2) in iteration $t$ of Algorithm~\ref{alg:Gen:scheduler}. Since all of $V_q$ completed before the start of phase $\tau$, we know that the set $A$ of unscheduled predecessors of $v_{q}$ is empty in iteration $t$ of Algorithm~\ref{alg:Gen:scheduler}. Therefore, we have that the set $A$ and machine $i$ satisfy all of (C1), (C3), and (C4). In this case, the algorithm places the long job on machine $i$, contradicting our assumption that $\tau \in \Phi$. 
\end{proof}

Finally, we define $f_i(v,\tau)$ to be the fraction of $v$ executed on machine $i$ in phase $\tau$. More formally, if $v$ does not execute on $i$, then $f_i(v,\tau) = 0$ for all $\tau$. Otherwise, let $t_s$ and $t_c$ be the start and completion times of $v$ on $i$. Then
\[ f_i(v,\tau) = \max\Big\{ \frac{\speed{i}(\min\{5\delay(\tau+1), t_c\} - \max\{5\delay\tau, t_s\})}{\proc{v}}, 0 \Big\}.
\]
We also define $f(v,\tau) = \max_i\{f_i(v,\tau)\}$.
Note that $f(v,\tau)$ ignores duplicate instances of job $v$, where $f_i(v,\tau)$ and $f_j(v,\tau)$ may both equal 1 if $v$ is duplicated on both machines. 
We prove the following two claims to establish properties of the function $f$. Inequality (\ref{claim:phase_load}) shows that Algorithm \ref{alg:Gen:scheduler} avoids duplicating jobs too many times. Equation (\ref{claim:job_completion}) shows that the function $f(v, \tau)$ represents the total fractional work done on job $v$ in phase $\tau$. 

\begin{lemma}
    \begin{align}
        \sum_{v\in V:\assign{v} \ge k} \proc{v} f(v,\tau) &\ge \frac{\log\log\delay}{\log \delay} \sum_{v \in V:\assign{v} \ge k} \sum_{i \in \group{k}} \proc{v} f_i(v,\tau) &\text{for all}~ \tau ~\text{and groups}~ \group{k}, ~\text{and}
        \label{claim:phase_load}
        \\
        \sum_{\tau} f(v,\tau) &= 1 &\text{for all jobs}~ v.
        \label{claim:job_completion}
    \end{align}
\end{lemma}

\begin{proof}
    We prove (\ref{claim:phase_load}) by induction on the number of iterations of line \ref{line:job_loop} in which some job $v$ such that $\assign{v} \ge k$ is placed on some machine. If there are no such iterations, then the claim follows from the fact that all jobs $v$ placed on $\group{k}$ must be such that $\assign{v} \ge k$.  
    Suppose the lemma holds up to $t$ iterations and consider iteration $t+1$. Let $f'(v,\tau)$ represent the fractional work on $v$ in the first $t$ iterations and $f'_i(v,\tau)$ define the fractional work of $v$ on $i$ for the first $t$ iterations. In iteration $t+1$, suppose some job $v$ such that $\assign{v} \ge k$ is placed on some machine. The job $\algofont{v} = v$ cannot have been scheduled earlier since it would have been added to either $\AlgoCurrent$ or $\AlgoComplete$. We also have that $A$ satisfies (C3) in iteration $t$ and that the jobs comprising at least a $\frac{\log\log\delay}{\log\delay}$ fraction of the total size of $A$ have not been placed on any other machine in a prior iteration. Finally, we have that $A$ satisfies (C4) in iteration $t$, so all elements of $A$ are assigned to higher indexed groups than $\group{k}$. So
    \begin{align*}
        \sum_{v:\assign{v} \ge k} \proc{v} f(v,\tau) &\ge \proc{v}f_j(v,\tau) + \frac{\log\log\delay}{\log\delay}\setproc{A} + \sum_{v:\assign{v} \ge k} \proc{v} f'(v,\tau)
        \\
        &\ge \proc{v}f_j(v,\tau) + \frac{\log\log\delay}{\log\delay}\setproc{A} + \frac{\log\log\delay}{\log\delay} \sum_{v:\assign{v} \ge k} \sum_{i \in \group{k}} f'_i(v,\tau) &\text{by induction}
        \\
        &\ge \frac{\log\log\delay}{\log\delay}\sum_{v:\assign{v} \ge k}\sum_{i \in \group{k}} f_i(v,\tau)
    \end{align*}
    where the last line follows trivially if $j \not\in \group{k}$.
    Inequality (\ref{claim:phase_load}) follows.
    
    We now prove (\ref{claim:job_completion}). By definition of Algorithm \ref{alg:Gen:scheduler}, all jobs that start and finish within a phase are not scheduled in any other phase. By Lemma \ref{lem:long_job_location}, those jobs that extend over multiple phases do so on a single machine. 
    Equation (\ref{claim:job_completion}) follows.
\end{proof}
    
\begin{theorem}[{\bf Makespan approximation}]
    There is a polynomial time algorithm that, given an instance of the DAG scheduling with fixed communication delay problem, computes a schedule whose makespan is $O(\log m \log \delay/ \log \log \delay)(OPT + \delay)$, where $OPT$ is the optimal makespan for the given instance.
\end{theorem}

\begin{proof}
    \david{set $\omega$ to $1 - (\log\log\delay/\log\delay)$}
    For a given instance $I$, let $\widehat{C}$ be the schedule output by Algorithm~\ref{alg:Gen:scheduler} and let $\optmakespan$ be the optimal makespan of $I$.
    Recall that we derived the group assignment $\assignfunc$ from the solution to \NCP{}{\guess}, where $\guess = 6\optmakespan$.
    Let $R$ be the highest index of any non-empty band of the solution to \NCP{}{\guess}. We claim that
    \begin{equation}
        \widehat{C} \le  \frac{20 \cdot KR\delay\log\delay}{\log\log\delay} + 5 \cdot \sum_{v \in \chain} \frac{\proc{v}}{\groupspeed{\assign{v}}} +   \frac{5 \log\delay}{\log\log\delay} \sum_{k = 1} ^K \frac{\setproc{\{v : \assign{v} = k \}}}{\groupsize{k}\groupspeed{k}} + \phaselength.
        \label{claim:schedule_bound}
    \end{equation}
    The proof of the claim is below. We now show that proving (\ref{claim:schedule_bound}) is sufficient to prove the theorem.
    We first show that $R\delay \le 4(\guess+\delay)$.
    %For any job $v$, if $v \in \band{R}$, then $R\delay \le \delay + 4\start{v}$. 
    For any job $v \in \band{R}$, we have that $\start{v} \ge \frac{\delay(R-1)}{4}$ by definition of $\band{R}$. So
    $R \delay = \delay + 4\frac{\delay(R-1)}{4} \le \delay + 4\start{v} \le 4(\guess + \delay)$ by Constraints (\ref{LP:Gen:execution}), (\ref{LP:Gen:makespan}), and (\ref{LP:guess}). So the first term of (\ref{claim:schedule_bound}) is $O(K \log \delay/\log\log\delay) (\guess +\delay)$.
    By Lemma \ref{lem:ChainBound}, the second term is $O(\guess)$.
    By Lemma \ref{lem:LoadBound}, the third term is $O(K \guess \log\delay/\log\log\delay)$. 
    Recalling that the number of machine groups is $K=O(\log m)$, this yields 
    \begin{align*}
        \widehat{C} &= 
        O(K (\log \delay /\log\log\delay) + K + K (\log \delay /\log\log\delay)) (\guess + \delay) + O(\delay)
        \\
        &= O(\log m \log \delay/\log\log\delay)  (\optmakespan + \delay) &\text{by definition of $\guess$.}
    \end{align*}
    Therefore, in order to prove the theorem, it is sufficient to prove (\ref{claim:schedule_bound}). 
    
    By definition of $\Phi$ and $\Phi_{\chain}$, we have that $\widehat{C} \le \phaselength|\Phi| + \phaselength|\Phi_{\chain}|$.
    By Lemma \ref{lem:long_job_location} all jobs in the chain are executed only on a single machine in their assigned groups.
    So, the time spent in $\sigma$ executing the chain $\chain$ is no more than $\sum_{v \in \chain} \frac{\proc{v}}{\groupspeed{\assign{v}}}$, by definition of $\groupspeed{k}$, and the number of phases in $\Phi_{\chain}$ is at most $\frac{1}{\delay} \sum_{v \in \chain} \frac{\proc{v}}{\groupspeed{\assign{v}}}$. So, all that remains to be shown is that 
    \begin{equation}
        \phaselength |\Phi| \le 20 \cdot K R \delay \log \delay/\log\log\delay  + \frac{5 \log\delay}{\log\log\delay} \sum_{k = 1} ^K \frac{ \setproc{\{v : \assign{v} \ge k\}}}{\groupsize{k}\groupspeed{k}} + \phaselength. 
        \label{eq:height_and_load}
    \end{equation}
    
    We partition $\Phi$ into $K+1$ sets. The first set, $\Phi_H$, is the set of height phases in $\Phi$. Each other set, $\Phi_L^k$, is the set of load phases in $\Phi$ in which $\group{k}$ is the slowest group such that $\tau$ is a load phase of $\group{k}$.
    By definition of $\Phi_H$ and $\Phi_L^k$, we have that $|\Phi| \le |\Phi_H| + \sum_k |\Phi_L^k|$. Therefore, the following two claims are sufficient to prove (\ref{eq:height_and_load}).
    \begin{align}
        \sum_k |\Phi_{L}^k| &\le \frac{\log\delay}{\log\log\delay} \sum_{k} \frac{\setproc{\{v:\assign{v} = k}}{\delay\groupsize{k}\groupspeed{k}}.
        \label{claim:load_phase_bound}
        \\
        |\Phi_H| &\le 4 K R (\log \delay/\log\log\delay) + 1. 
        \label{claim:height_phase_bound}
    \end{align}
    We now prove claims (\ref{claim:load_phase_bound}) and (\ref{claim:height_phase_bound}).
    
    \textit{Proof of (\ref{claim:load_phase_bound}).}
    Claim (\ref{claim:load_phase_bound}) follows from the following inequalities, which we prove below.  
    \[ \sum_{k' \ge k} |\Phi_{L}^{k'}| 
    %\le \frac{\setproc{\{v:\assign{v} \ge k\}}}{\delay\sum_{k' \ge k} \groupsize{k'}\groupspeed{k'}} 
    \le \sum_{k' \ge k} \frac{\setproc{\{v:\assign{v} = k'}}{\delay\groupsize{k'}\groupspeed{k'}}. \]
    We first show that 
    \[\min_{\tau \in \Phi_L^k} \{\proc{v} f(v,\tau) \} \ge \delay\groupsize{k}\groupspeed{k}\cdot \frac{\log\log\delay}{\log\delay}.\]
    For arbitrary $\tau \in \Phi_L^k$, we have that all machines in $\group{k}$ are executing jobs for at least $\delay$ time in phase $\tau$. This yields
    \[ \delay\groupsize{k}\groupspeed{k} \le \sum_{i \in \group{k}} \sum_{v:\assign{v} \ge k} \proc{v} f_i(v,\tau) \le \sum_{v:\assign{v} \ge k} \frac{\log\delay}{\log\log\delay}\proc{v} f(v,\tau) \]
    by (\ref{claim:phase_load}). 
    For all jobs $v$ scheduled on groups $\group{k}, \ldots, \group{K},$ we have $\assign{v} \ge k$, 
    Also, by (\ref{claim:job_completion}), we have that $\sum_{\tau} \sum_{v:\assign{v} \ge k} \proc{v} f(v,\tau) \le \setproc{\{v:\assign{v} \ge k}$. So
    \begin{align*}
        \sum_{k' \ge k} |\Phi_L^k| &\le \frac{\setproc{\{ v: \assign{v} \ge k \}}}{\sum_{k' \ge k} \min_{\tau \in \Phi_L^k} \{ \sum_{v:\assign{v} \ge k'} \proc{v} f(v,\tau)\}}
        \\
        &\le \frac{\log\delay}{\log\log\delay} \frac{\setproc{\{ v: \assign{v} \ge k \}}}{\sum_{k' \ge k} \delay \groupsize{k'}\groupspeed{k'}} \le \frac{\log\delay}{\log\log\delay} \sum_{k' \ge k} \frac{\setproc{\{v:\assign{v} = k'}}{\delay\groupsize{k'}\groupspeed{k'}}.
    \end{align*}
    This proves claim (\ref{claim:load_phase_bound}).
    
    \textit{Proof of (\ref{claim:height_phase_bound}).}
    For simplicity, we consider each band of the solution to \NCP{}{\guess}, and partition its jobs that belong to $\bigcup_q V_q$ into \textit{families}.  Formally, we define family $F_{r,d}$ to be the set of jobs $v \in \band{r} \cap \bigcup_q V_q$ such that $(d-1)\delay\groupspeed{\assign{v}} < \setproc{\predex{v} \cap \band{r}} \le d\delay\groupspeed{\assign{v}}$.
    Families allow us to more easily reason about which jobs are available to be scheduled at a given step of the algorithm. Because we require in (C1) at line \ref{line:conditions} that the set $A$ take no longer than $\delay$ to execute on the machine $\algofont{i}$, there may be jobs in the lowest band that cannot be placed on the machine. However, any job in the lowest family of the lowest band can be placed, and we will reason that Algorithm~\ref{alg:Gen:scheduler} makes progress on this family in each height phase.  
    By Lemma \ref{lem:Gen:HeightBound} there are at most four non-empty families per band, so we lose only a constant factor by simplifying our analysis in this way. 

    Suppose $\tau \in \Phi_H$ and phase $\tau$ is not the last phase in $\sigma$. By Lemma \ref{lem:height_phase_limit}, for some $q$, there is a job in $V_q$ that is not scheduled by the end of phase $\tau$. We fix $V_q$ to be the lowest indexed such set. Let $\band{r}$ be the lowest indexed band containing an unscheduled job of $V_q$ and let $F_{r,d}$ be the lowest $d$-indexed family of $\band{r}$ containing an unscheduled job of $V_q$. Let $k$ be the index of the slowest group with an unscheduled job $v$ in $F_{r,d}$ and $i$ some machine in group $\group{k}$ that executes jobs for less than $\delay$ time in phase $\tau$.  
    By definition of the algorithm, scheduling $v$ on $i$ in phase $\tau$ must have violated one of the conditions (C1) through (C4). If $d=1$ then it is clear by definition of $\band{r}$ and $F_{r,d}$ that (C1) is not violated. 
    Suppose $d >1$. Then all jobs in lower $d$-indexed families have already been started on some machines in previous phases. Since any member of any families takes less than $\delay$ time in $\sigma$, all such jobs have also been completed in previous phases. Therefore, the total size of unscheduled predecessors of $v$ is less than $\delay\speed{\assign{v}}$.
    Also, by definition of $i$, (C2) is not violated. 
    
    We now show that (C4) is not violated. First, we show that $v$ has no uncompleted predecessors that were started in a previous phase.  Suppose $v$ has some uncompleted predecessor $u$ started in a previous phase.
    %and assigned to a group slower than $\group{\assign{v}}$. 
    Since $\tau \in \Phi$, $u$ cannot be a member of the chain by Lemma \ref{lem:non_chain_phase_execution}. Then $u$ is some predecessor of $v$ which completes after $v_{q-1}$ (or precedes $v_1$ if $q=1$) which contradicts the construction of the chain. 
    Therefore, all predecessors of $v$
    that were started in previous phases are completed by time $\phaselength\tau + \delay$ and their results communicated to all machines by time $\phaselength\tau + 2\delay$. So, suppose that $v$ has some uncompleted predecessor $u$ assigned to a group slower than $\group{k}$. This constradicts $k$ being the index of the slowest group with an unscheduled job in $V_q$.  Therefore, (C4) is not violated. 
    So it must be that (C3) is violated.  
    
    We now show that in $\log \delay/\log\log \delay$ height phases after phase $\tau$ all jobs in $F_{r,d}$ assigned to group $\group{k}$ are scheduled.
    Let $A_{\ge\tau}$ be the set of predecessors of $v$ started in phase $\tau$ or later.
    Since there are no predecessors of $v$ still executing from previous phases, $A_{\ge\tau}$ corresponds to the set $A$ in Algorithm \ref{alg:Gen:scheduler} when the algorithm is scheduling phase $\tau$. 
    Let $A_{\tau}$ be the set of predecessors of $v$ executed during phase $\tau$. The violation of (C3) entails that $\setproc{A_{\ge\tau} \cap A_{\tau}} \ge (1-\log\log\delay/\log\delay) \setproc{A_{\tau}}$, and so size of the set $A_{\ge \tau}$ of unfinished predecessors reduces by a factor of $\log\delay$ with each height phase $\tau$. By definition of $F_{r,d}$, we have that $\setproc{A_{\ge\tau}} \le \delay\groupspeed{k}$.
    So, by our scaling of speeds, in at most $\log_{\log\delay}(\delay \groupspeed{k}) \le \log_{\log\delay}(\delay\speed{m}) \le \log_{\log\delay}(\delay) = \log\delay/\log\log\delay$ height phases, we have that the set of uncompleted predecessors of $v$ has total size at most 1. 
    By our scaling of job sizes, the smallest job has size at least 1, so in $\log \delay/\log\log\delay$ height phases after phase $\tau$, we have that $v$ is scheduled. Therefore, every job in $F_{r,d}$ assigned to $\group{k}$ is scheduled in at most $\log \delay/\log\log\delay$ height phases after phase $\tau$. So, every job in $F_{r,d}$ assigned to any speed is scheduled in at most $K \log \delay/\log\log\delay$ height phases after $\tau$. Since there are four families per band, the entire band $\bigcup_{d=1}^4 F_{r,d}$ is scheduled in at most $4K\log \delay/\log\log\delay$ height phases after $\tau$. By definition of $R$ we have that $R \ge \max \{r : \band{r} \cap \bigcup_q V_q \ne \varnothing \}$, i.e.\ the highest band index is larger than the highest index of any band containing a job in $\bigcup_q V_q$.
    
    The above argument proves that all jobs in sets $V_q$ are completed after $4K\log\delay/\log\log\delay$ height phases. By Lemma \ref{lem:height_phase_limit}, once all $V_q$ have been completed, there are no further height phases in $\sigma$ except possibly for the last phase. 
    Therefore, there are at most $4RK\log \delay/\log\log\delay + 1$ height phases in $\sigma$. 
    This proves claim (\ref{claim:height_phase_bound}).
\end{proof}

==> Old Makespan/compute_schedule.tex <==
In this section, we describe the subroutine that outputs a schedule $\sigma$ for a given instance $(G,M,\delay)$ and assignment of each job to a group of machines in $M$. 
%We divide the section into two parts. \ref{sec:final_scheduler} presents of the subroutine and proves some of its basic properties. \ref{sec:final_analysis} relates the makespan of $\sigma$ output by the subroutine to the optimal makespan  of $\instance$. We assume the group assignment was derived as in Section~\ref{sec:group_assign} from a feasible solution to \NCP{}{\guess} for $\guess = 6\optmakespan$.
%\subsubsection{The Subroutine}
In the following, we refer to a \textit{phase} $\tau$ of the schedule $\sigma$ to be the span of time $[\phaselength\tau,\phaselength (\tau+1))$. 
Our algorithm builds on ideas used in the scheduling algorithms given in \cite{LR02} and \cite{chudak1999approximation}. We apply the phase-by-phase approach used in \cite{LR02} to decide in which phase a job (and all its remaining predecessors) starts its execution. However, unlike \cite{LR02}, our algorithm accounts for arbitrarily slow machines and arbitrarily large jobs, both of which may cause a job's execution to last well beyond the end of the phase in which it started. As in \cite{chudak1999approximation}, we use the group assignment to guide where jobs are scheduled. One fundamental difference between our algorithm and that in \cite{chudak1999approximation} is that, given certain conditions, we allow a job to be scheduled on machines in groups to which the job is not assigned.

\begin{algorithm}
\KwData{problem instance $(G,M,\delay)$, assignment $\assignfunc$ of jobs to groups, and overlap parameter $\omega \le 1$}
\KwResult{a schedule $\sigma$ of $G$ on $M$}
    $\sigma \leftarrow (\bot)_{n,m}$ \label{line:schedule_initialize}\;
    $T_1, \ldots, T_m \leftarrow 0$ \tcp*{track completion times of last jobs on machines}
    $\tau \leftarrow 0$ \tcp*{tracks index of current phase}
    $\AlgoCurrent \leftarrow \varnothing$ \tcp*{tracks the jobs currently being executed on machines}
    $\AlgoComplete \leftarrow \varnothing$ \tcp*{tracks the jobs that have been completed}
    $\leads \leftarrow \varnothing$ \tcp*{stores special job-machine pairs (for analysis)}
    %$\omega \leftarrow 1 - (\log\log\delay/\log\delay)$ \tcp*{defines the maximum amount of overlap allowed}
    \While{there is some job $v^*$ such that, for all machines $i$, $\sigma[v^*, i] = \bot$ \label{line:job_loop}}{
        $\AlgoCurrent \leftarrow \AlgoCurrent \setminus \AlgoComplete$\;
        \ForAll{$k \in \{1,\ldots,K\}$}{
                $U_{k} \leftarrow \{v: \assign{v} \ge k \} \setminus \AlgoComplete$\;
        }
        \ForAll{$i \in M$}{
            $T_{i} \leftarrow \max\{ T_{i}, \phaselength\tau + 2\delay \}$ \label{line:Ti_update}\;
        }
        \ForAll{$k \in \{1,\ldots,K\}$ \label{line:group_loop}}{
            \ForAll{$v \in V \setminus (\AlgoCurrent \cup \AlgoComplete)$ such that $\assign{v} = k$ \label{line:assigned_jobs_loop}}{
                $A \leftarrow \predex{v} \setminus \AlgoComplete$ \label{line:A_def}\;
                $i \leftarrow \argmin_j \{T_j : j \in \group{k} \}$ \label{line:i_def}\;
                \If{(C1) $\setproc{A} \le \delay\speed{i}$ and (C2) $\setproc{A \cap \AlgoCurrent} \le \omega \cdot \setproc{A}$ and (C3) $A = A \cap U_{k}$  \label{line:conditions}}{
                    $\leads \leftarrow \leads \cup \{(v,i)\}$\;
                    \ForAll{$u \in A \cup \{ v \}$ in topological order \label{line:ancestor_loop}}{
                        \If{$\sigma[u,i] = \bot$}{
                            $\sigma[u,i] \leftarrow T_{i}$ \label{line:start_time}\;
                            $T_{i} \leftarrow T_{i} + \proc{u}/\speed{i}$ \label{line:add_to_Ti}\;
                            $\AlgoCurrent \leftarrow \AlgoCurrent \cup \{ u \}$\label{line:add_to_current}\;
                        }
                    }
                }
            }
        } 
        $\tau \leftarrow \max \big\{ \tau + 1, \min_i \{ \floor{T_i/\phaselength} \} \big\}$ \label{line:phasevar_update}\;
        $\AlgoComplete \leftarrow \AlgoComplete \cup \{ v : v ~\text{finishes by time}~ \phaselength\tau + \delay \}$ \label{line:completed_update}\;
    }
    \Return $\sigma$\;
\caption{Phase-Structured Group-Based Scheduling}
\label{alg:Gen:scheduler}
\end{algorithm}

\vfill

\begin{figure}
    \centering
    \includegraphics{Figures/phase_structure_3rho_overflow.pdf}
    \caption{Phase $\tau$ of a schedule output by Algorithm \ref{alg:Gen:scheduler}. The machines are listed vertically on the left and time proceeds from left to right. For each dark gray job on machine $i$, the pair $(v,i)$ is an element of $\leads$ at the completion of Algorithm \ref{alg:Gen:scheduler}. All other jobs are shown in light gray. All machines except for machine 4 are busy for at least $\delay$ time in this phase.}
    \label{fig:phase_structure}
\end{figure}

\david{I have changed the length of each phase to $4\delay$ and removed one condition (formerly (C2)) that checked whether the current machine $i$ had less than $\delay$ load in the current phase.}

The subroutine is explicitly stated as Algorithm~\ref{alg:Gen:scheduler} which we now describe informally.
Algorithm~\ref{alg:Gen:scheduler} takes as input an instance $(G, M, \delay)$, as well as an assignment $\assignfunc:V \to \{1,\ldots,K\}$ of jobs to groups, where groups are defined as in Section \ref{sec:group_assign}.
It constructs the schedule $\sigma$ phase-by-phase. In scheduling a given phase, the algorithm iterates sequentially through each group $\group{k}$ and through each job $v$ such that $\assign{v} = k$. The algorithm schedules $v$ in phase $\tau$ on a machine $i$ in group $\group{k}$ if the following conditions are met. 

First (C1), the algorithm checks if the total size of $v$'s uncompleted predecessors is small enough. This ensures that, if $v$ is scheduled on $i \in \group{k}$ and takes more than $\delay$ time to complete, then $\assign{v} = k$. 
%Second (C2), the algorithm checks that the current last job on $i$ ends before time $\phaselength\tau + 3\delay$. If machine $i$ is already executing jobs for $\delay$ time this phase then we consider $i$ to be doing a sufficient amount of work and choose not to schedule more jobs on it. This is done to ensure that all jobs start early enough to have sufficient work done on them during the phase. 
Second (C2), the algorithm checks that the total size of $v$'s predecessors already scheduled in phase $\tau$ is less than $\omega$ times the total size of $v$'s uncompleted predecessors.
%This check allows us to prove two things about the resulting schedule. 
This ensures that there is a sufficient amount of non-redundant work on each machine.
Third (C3), the algorithm checks that all of $v$'s remaining predecessors have been assigned to higher indexed groups. This check allows us to infer that, for any $k$, the total number of jobs executed on groups $\group{k}, \ldots, \group{K}$ is no more than the total number of jobs assigned to those groups. 
%Since the capacities decrease as indices increase total capacity of group $\group{k}$ is larger than all higher indexed groups, such phases can only happen a few times before all jobs assigned to faster groups have been completed.

Figure \ref{fig:phase_structure} shows how Algorithm \ref{alg:Gen:scheduler} structures each phase. 
The first $\delay$ time units of the phase are used to execute any jobs that have not completed from previous phases.
The next $\delay$ time units are used to communicate the results of any jobs that finished before time $\phaselength\tau + \delay$. 
%All jobs scheduled in phase $\tau$ begin between times $\phaselength\tau + 2\delay$ and $\phaselength(\tau + 1)$.
The last $\delay$ time units of the phase are used to start executing any jobs scheduled in phase $\tau$, though the algorithm may schedule beyond phase $\tau$ on any machine before updating its phase index variable. 

%We now prove several lemmas that establish some basic properties of Algorithm \ref{alg:Gen:scheduler} and the output schedule $\sigma$.

\begin{lemma}[{\bf Polynomial running time}]
    Algorithm \ref{alg:Gen:scheduler} runs in time polynomial in $n$ and $m$. % $O(n^3m)$.
\end{lemma}

\begin{proof}
    We prove that the while-loop at line \ref{line:job_loop} iterates at most $O(nm)$ times. The polynomial runtime of all other instructions can be checked easily.
    
    We show that if, at any point in the run of Algorithm \ref{alg:Gen:scheduler}, $\algofont{\phasevar} = \tau$, then either some job starts or completes in phase $\tau$ of $\sigma$. In the first iteration of the outer while-loop, we have $\phasevar = 0$. We can see that some job starts in phase 0 by noting that any job $v$ such that $\predex{v} = \varnothing$ meets all conditions (C1) through (C4) for any $i \in \group{\assign{v}}$. So we suppose that, in iteration $t$ of the outer while-loop, $\algofont{\phasevar}$ has been updated to $\tau$ by line \ref{line:phasevar_update} in the previous iteration. If, for some $i$,  $\algofont{\phasevar}$ was updated to $\floor{T_i/\phaselength}$ then we have that some job on machine $i$ completes in phase $\tau$. 
    So suppose that the previous iteration of the while-loop we had  $\algofont{\tau} = \tau-1$. In this case, we know that all jobs scheduled prior to the start of phase $\tau$ on all machines completed by time $\phaselength\tau$. Therefore, by time $\phaselength\tau + \delay$ all machines have completed their jobs and have had time to communicate their results to all other machines. If there were no remaining jobs to schedule, then the while-loop would not have iterated by the continuation condition. So, there is some job $v$ that has not yet been scheduled, all of whose predecessors have been scheduled in previous phases with their results communicated to all machines. Therefore, job $v$ satisfies constraints (C1) through (C4) for any machine in $\group{\assign{v}}$. Therefore, either $v$ or some other job is started in phase $\tau$. 
    
    Since a job is started or completed for every value of $\algofont{\phasevar}$, and each job is duplicated at most $m$ times, there are at most $2nm$ iterations of the outer-while loop. 
\end{proof}

%The next lemma shows that any job $v$ with a copy whose execution in $\sigma$ takes longer than the communication delay is executed in its group and on exactly one machine. From now on, we use ``step'' to describe the execution of an instruction in the algorithm and reserve ``time'' for time in the schedule $\sigma$.

From here on, we refer to jobs whose execution takes longer than time $\delay$ in $\sigma$ as {\em long} jobs. The following lemma entails that each long job $v$ has exactly one copy in $\sigma$ and is scheduled on some machine in its assigned group.

\begin{lemma}[{\bf Long jobs scheduled on unique machine in assigned group}]
    If Algorithm \ref{alg:Gen:scheduler} schedules job $v$ on machine $i$ and $\proc{v} > \delay\speed{i}$, then $i \in \group{\assign{v}}$ and Algorithm \ref{alg:Gen:scheduler} schedules $v$ on no other machines $j \ne i$.
    \label{lem:long_job_location}
\end{lemma}

\begin{proof}
    Suppose Algorithm~\ref{alg:Gen:scheduler} schedules job $v$ on machine $i$ and $\proc{v}/\speed{i} > \delay$. We show that $(v,i)$ is an element of $\leads$ at the completion of Algorithm~\ref{alg:Gen:scheduler}, which entails that $i \in \group{\assign{v}}$. Suppose $(v,i) \not\in \leads$. Consider the iteration $t$ of line~\ref{line:job_loop} in which $v$ is scheduled on $i$. In this iteration, $v \in A$ with $A$ defined for some $u$ that is added to $\leads$ in iteration $t$. However, in this case, $\setproc{A} > \delay\speed{i}$ by supposition. Therefore, $(v,i) \in \leads$.
    
    We now consider whether Algorithm~\ref{alg:Gen:scheduler} places $v$ on any other machine. Let $t$ be the iteration of line~\ref{line:job_loop} in which $v$ is scheduled on $i$. First, suppose that $v$ is placed on $j \ne i$ in some iteration prior to $t$. In this case, during iteration $t$ $v$ would be an element of either $\AlgoCurrent$ or $\AlgoComplete$ and so $(v,i)$ could not be added to $\leads$ in iteration $t$, violating our reasoning above. So, suppose that $v$ is placed on some $j \ne i$ in an iteration $t' < t$. Since $v$ was placed on $i$ in iteration $t$, it is an element of $\AlgoCurrent$ (by line \ref{line:add_to_current}) in $t'$ and so $(v,i)$ cannot be the pair added to $\leads$ in $t'$. So $v \in A$ in iteration $t'$.
    We now run through case analysis. If $j \in \group{k}$ for $k > \assign{v}$, then $A \cap U_k \ne A$, and so $A$ does not satisfy (C3). So we suppose that $j \in \group{k}$ for $k \le \assign{v}$. Since $v$ is scheduled on $j$, we have that $A$ satisfies (C1) and so $\setproc{A} \le \delay\speed{j}$. Since $\proc{v} > \proc{v} \speed{j} \ge \omega \cdot \proc{v} \speed{j}$, we have that $\setproc{A \cap \AlgoCurrent} > \omega \setproc{A}$. Therefore, (C2) is violated. The lemma follows.
\end{proof}



\junk{
The next lemma shows that the starting times of all jobs in a phase fall within a $2\delay$ window.

\begin{lemma}[{\bf Start times in a phase fall in a $2\delay$ interval}]
    For any phase $\tau$ of the schedule output by Algorithm \ref{alg:Gen:scheduler}, all jobs started in phase $\tau$ have their starting times between $\phaselength\tau + 2\delay$ and $\phaselength\tau + 4\delay$.
    \label{lem:start_times}
\end{lemma}

\begin{proof}
    Consider the first job $v$ placed on machine $i$ in phase $\tau$. By the update of $T_i$ at line \ref{line:Ti_update}, we have that the start time of $v$ is at least $\phaselength\tau + 2\delay$. So consider the last job  $u$ placed on machine $i$ in phase $\tau$ and suppose it was placed at step $t$ of Algorithm \ref{alg:Gen:scheduler}. Since $u$ is the last job placed on $i$, when it is placed we have that $\algofont{v} = u$ and that $A$ satisfies conditions (C1) and (C2) at step $t$. By the satisfaction of (C1), we have that $\setproc{A} \le \delay\speed{i}$. By the satisfaction of (C2) we have that $T_i < \phaselength\tau + 3\delay$ before any of $A$ is placed on machine $i$. Since all jobs are placed immediately after each other (by lines \ref{line:start_time}, \ref{line:add_to_Ti}) this entails that the start time of $u$ is less than $\phaselength\tau + 4\delay$.  
\end{proof}
}

\begin{lemma}[{\bf Correctness of schedule}]
    Algorithm \ref{alg:Gen:scheduler} outputs a valid schedule. 
\end{lemma}

\begin{proof}
    We show first that precedence relations are maintained for all jobs scheduled within a phase.  This follows from the fact that, for any job $v$ scheduled to start within a phase, $v$ and all its previously unscheduled predecessors are scheduled in topological order on the same machine. 
    We now show that precedence relations are maintained across phases. If job $v$ along with the set $A \subseteq \predex{v}$ is started in phase $\tau$ on some machine $i$, then all remaining predecessors were started in previous phases. If these remaining predecessors completed in those phases, then the precedence constraints are satisfied. If some predecessor $u$ does not complete in the phase where its starts then, by Lemma~\ref{lem:long_job_location} and the assignment of $A$ at line \ref{line:A_def}, $v$ cannot begin until $u$ has completed.
    Finally, we show that the communication delay condition is met. Suppose a job $v$ starts its execution in phase $\tau$ and is placed at step $t$. Then we know that all predecessors not in $\AlgoComplete$ at step $t$ are duplicated on the same machine as $v$ and that all predecessors in $\AlgoComplete$ at step $t$ complete their execution by time $\phaselength\tau + \delay$.  By Lemma we have that the start time of $v$ is after time $\phaselength\tau + 2\delay$. Therefore, the communication delay constraint is satisfied.
\end{proof}

==> Old Makespan/efficiency.tex <==
Algorithm is polynomial time, but uses ellipsoid method.
If we hold delay $\delay$ as a fixed constant, then we can eliminate use of ellipsoid method. In this case, as the number of jobs $n$ gets large, there are at most $n$ choose $\delay\speed{m}$ constraints. Since we can treat $\speed{m} = 1$ by our normalization, this results in $n$ choose $\delay = O(n^{\delay})$ delay constraints. 

Motivate this assumption. 

Discuss Kulkarni et al, who assume the number of machines $m$ is fixed and all communication delays are upper bounded by a constant. 

==> Old Makespan/group_assignment.tex <==
In this section, we present the third subroutine of our algorithm. For a given instance $I = (G,M,\delay)$ and a feasible solution of \NCP{}{\guess}, this subroutine assigns each job to a subset of machines in $M$. Per Lemmas~\ref{lem:elim_slow} and \ref{lem:MP_solution}, let $\guess$ equal $6 \optmakespan$,
and suppose, for each $i \in M$, $\speed{i} \ge \speed{m}/m$.

The first step of the subroutine is to partition the set of machines $M$ into $K + 1$ groups, $\group{1}, \ldots, \group{K}$. 
%We define group $\group{0}$ to be the set of machines $i \in M$ such that $\speed{i} \le \speed{m}/m$, where machine $m$ is the fastest machine in $M$. 
We define $\group{k}$ to be the set of all machines $i$ such that $\speed{i} \in (2^{(k-1)-\log(m)},2^{k-\log(m)}]$. We define $\groupsize{k}$ to be the number of machines in $\group{k}$ and $\groupspeed{k}$ to be the speed of the slowest machine in group $\group{k}$. Since the speeds of all machines are within a factor of $m$, we have that $K = \log m$. Recall that the fastest machine in $M$ has speed 1.

We define the group assignment $\assignfunc : V \to \{1,\ldots,K\}$ as follows.
%We can then use Lemma~\ref{lem:MP_solution} and Appendix~\ref{sec:elim_slow_machines} to find a feasible solution to $\MPGuess{\canoninstance}$ with variables $\LPind{v}{i}, \start{v}, \comp{v}$, and $\LPmakespan$, where $\optmakespan$ is the optimal makespan for $\instance$. 
%Recall that group $k$ is the set of machines $i \in \canonmachines$ such that $\speed{i} \in  [2^{(k-1)-\log(m)},2^{k-\log(m)})$. 
Define $\med{v} = \min \{ k : \sum_{k' \le k} \sum_{i \in k'} \LPind{v}{i} \ge 1/2 \}$.
Then, for any $v$, 
\[ \assign{v} = \arg\max_k \Big\{ \sum_{i \in \group{k}} \speed{i} : k \ge \med{v} \Big\} . \]
Informally, $\assign{v}$ is the highest capacity group such that at least half of job $v$ is assigned to groups slower than $\group{k}$. 
%We say that a group $\group{k}$ is \textit{vacant} if $\{v:\assign{v}=k\} = \varnothing$.
\junk{We note that an alternative group construction is given in \cite{Li17} where the author reduces the approximation ratio of the algorithm in \cite{chudak1999approximation} from $O(\log m)$ to $O(\log m /\log\log m)$. The construction and assignment we give above gives us a factor of $O(\log m)$. However, given our analysis, we cannot apply the method of \cite{Li17} to similarly reduce our approximation ratio.
While our construction ensures that the speeds of all machines within a group are within a factor of 2 of each other, the construction of \cite{Li17} allows for these speeds to be off by up to a factor of $\log m/\log\log m$. 
If we were to use this alternate construction then this difference in speed we would give an additional factor of $O(\log m /\log\log m)$ in Lemma~\ref{lem:Gen:HeightBound} below, resulting in an overall approximation ratio of $O(\log ^2 m \log \delay/\log^2 \log m \log \log \delay)$. }
In the remainder of the section, we show properties of this assignment. Toward this end, we partition $V$ into sets called \textit{bands} where the elements $v$ of each band are determined by the value $\start{v}$.

\begin{definition}
    Band $\band{r}= \{v: \delay(r-1)/4 \leq \start{v} < \delay r/4\}$. 
    \label{def:band}
\end{definition}

In the following lemma, we show that, for any job $v$, the total size of $v$'s predecessors that occupy the same band is no more than the amount that can be completed in a constant number of communication phases on some machine in $v$'s assigned group.


\begin{lemma}[{\bf Upper bound on processing time of predecessors of a job in a band}]
    For any job $v \in \band{r}$, we have $\setproc{\band{r} \cap \predex{v}} < 4\delay \groupspeed{\assign{v}}$.
\label{lem:Gen:HeightBound}
\end{lemma}

\begin{proof}
    We fix $v$ and let $A = \band{r} \cap \predex{v}$.
    We also fix the machine $i$ to be the lowest indexed machine such that $\sum_{j \le i} \LPind{v}{j} \ge 1/2$. By definition of the groups, if $i \in \group{k}$ then $k \le \assign{v}$. In this case, $\speed{i} < 2\groupspeed{\assign{v}}$ and it is sufficient to show that $\setproc{A} \le 2\delay\speed{i}$.
    
    Suppose, for the sake of contradiction, that $\setproc{A} > 2\delay \speed{i}$. If there is any $u \in A$ with $\proc{u} \ge \delay\speed{i}$, then
    \[ \start{u} > \start{v} - \frac{\delay}{4} \ge \start{v} - \frac{\delay}{2} \sum_{j \le i} \LPind{v}{i} \]
    and so constraint (\ref{LP:Gen:large_size_height}) is violated. So we assume that all jobs $u \in A$ are such that $\proc{u} < \delay\speed{i}$, in which case $\trimproc{u}{i} = \proc{u}$.
    By definition of the machine assignment, we have $\sum_{j \le i} \LPind{v}{j} \geq 1/2$. By definition of $\band{r}$, we have that $\start{v} < \delay r/4$ and $\start{u} \ge \delay (r-1)/4$ for all $u \in A$. So, for all $u\in A$,
        \begin{equation*}
        \start{v} - \frac{\delay}{2} \sum_{j \le i} \LPind{v}{j} ~<~ \frac{\delay r}{4} - \frac{\delay}{4} ~\le~ \start{u},
        \end{equation*}
    which contradicts (\ref{MP:height}).
\end{proof}

Although we can upper bound the size of a job's predecessor set within a band, there is no limit on the total amount of work that can be put on a single band. For example, if all jobs are independent, then the solution to \NCP{}{\guess} might place all jobs on the first band. The following lemma, due to \cite{chudak1999approximation}, addresses this issue by providing a lower bound on the optimal LP solution in terms of the total load across all groups. We repeat the lemma and provide a proof for our  program.

\begin{lemma}[{\bf \cite{chudak1999approximation} Lower bound on $\guess$ in terms of load}]
\[
    \sum_{k=1}^K \frac{\setproc{\{v : \assign{v} = k\}}}{\groupsize{k}\groupspeed{k}} \le 2K\guess.
    \]
    \label{lem:LoadBound}
\end{lemma}

\begin{proof}
     Let $y_{v,k} = 1$ if $\assign{v} = k$ and 0 otherwise, for all $v \in V$ and $k = 1,\ldots,K$. Then, by definition of the group assignment, the set of all variables $y_{v,k}$ gives an optimal solution to the following linear program. 
    \begin{align}
        \min ~ \sum_{k=1}^K \sum_{v \in V} \frac{ \proc{v} y_{v,k}}{\sum_{i \in \group{k}} \speed{i}}
        \label{sim:objective}
        \\
        \text{s.t.} \quad \sum_{k=1}^K y_{v,k} &= 1 &\text{for all}~ v \in V, k = 1,\ldots,K
        \label{sim:cover}
        \\
        y_{v,k} &= 0 &\text{for all}~ v \in V, k = 1,\ldots, \med{v}-1
        \label{sim:slow}
        \\
        y_{v,k} &\ge 0 &\text{for all}~ v \in V, k = 1,\ldots,K
        \label{sim:nonneg}
    \end{align}
    We give a feasible solution to this linear program whose objective values is at most $2K\guess$, thereby proving the lemma. 
    
    Let $\LPind{v}{i}, \start{v}, \comp{v},$ and $\LPmakespan$, for all $v \in V$ and $i \in M$, represent the variables in the the feasible solution to \NCP{}{\guess}. 
    %For all jobs $v$, let $\beta_v = \sum_{k = \med{v}}^K \sum_{i \in \group{k}} \LPind{v}{i}$. 
    Then, for all jobs $v$ and groups $\group{k}$, we set $y_{v,k}$ as follows.
    \[ y_{v,k} \leftarrow 
    \begin{cases}
        0 &\text{if}~ k < \med{v}
        \\
        \sum_{i\in \group{k}} \LPind{v}{i} \big/ \sum_{k = \med{v}}^K \sum_{i \in \group{k}} \LPind{v}{i} &\text{otherwise.}
    \end{cases}\]
    It is easy to see that this assignment satisfies all constraints (\ref{sim:cover}), (\ref{sim:slow}), and (\ref{sim:nonneg}). We show that the objective (\ref{sim:objective}) is no more than $2K\guess$.
    \begin{align*}
        \sum_{k=1}^K ~ \sum_{v \in V} ~ \frac{ \proc{v} y_{v,k}}{\sum_{i \in \group{k}} \speed{i}} %&= \sum_{k=1}^k \sum_{v \in V: \med{v} \le k} \frac{ \proc{v} y_{v,k}}{\groupsize{k}\groupspeed{k}} &\text{by definition of}~ \med{v}
        %\\
        &\le \sum_{k=1}^k ~ \sum_{v \in V: \med{v} \le k} \frac{ \proc{v} \sum_{i \in \group{k}} \LPind{v}{i}}{\groupsize{k}\groupspeed{k} \sum_{k = \med{v}}^K \sum_{i \in \group{k}} \LPind{v}{i}} &\text{by assignment of}~ y_{v,k}
        \\
        &\le \sum_{k=1}^k ~ \sum_{v \in V: \med{v} \le k} \frac{  \guess} {\sum_{k = \med{v}}^K \sum_{i \in \group{k}} \LPind{v}{i}} &\text{by Constraint~(\ref{LP:Gen:load})}
        \\
        &\le \sum_{k=1}^k 2 \guess = 2K\guess &\text{by definition of $\med{v}$.}
    \end{align*}
    The lemma follows.
\end{proof}

We note that an alternative group construction is given in \cite{Li17} where the author reduces the approximation ratio of the algorithm in \cite{chudak1999approximation} from $O(\log m)$ to $O(\log m /\log\log m)$. \junk{The construction and assignment we give above gives us a factor of $O(\log m)$.} However, given our analysis, we have been unable to apply the method of \cite{Li17} to similarly reduce our approximation ratio.
While the speeds of all machines within a group in our algorithm are within a factor of 2 of each other, the construction of \cite{Li17} allows for these speeds to be off by up to a factor of $\log m/\log\log m$. 
Use of this alternate construction incurs an additional factor of $O(\log m /\log\log m)$ for the upper bound proved in Lemma~\ref{lem:Gen:HeightBound} on the processing time of a job's predecessors in a band, resulting in a worse approximation ratio than our current bound. 

==> Old Makespan/makespan_intro.tex <==
Our algorithm for minimizing makespan is based on linear and non-convex programming relaxations of the problem. In Section \ref{sec:lp}, we present our linear and non-convex programs. We prove that there exist feasible solutions to the non-convex program that lower-bound the optimal linear program solution, and that these solutions also lower bound the optimal makespan. Building on these programs, our algorithm has four subroutines which we outline here. 
The first subroutine takes as input a given instance $I$ of DAG scheduling with fixed communication delay, and preprocesses the instance to remove any excessively slow machines.
The second subroutine, presented in Section \ref{sec:LP_solve}, takes as input any instance of the problem and finds a feasible solution to the non-convex program that lower bounds the optimal linear program solution. 
The third subroutine, presented in Section \ref{sec:group_assign}, takes as input a feasible solution to the non-convex program and derives an assignment of each job to some group of machines. 
The fourth subroutine, presented in Section \ref{sec:scheduler}, takes as input an instance $(G,M,\delay)$ and an assignment of its jobs to groups of machines, and computes start times for each job on some set of machines (not necessarily the ones to which it is assigned). This final subroutine outputs a complete schedule.  
%This final subroutine outputs a schedule of all jobs on the remaining machines, which also serves as a schedule for the original instance. 

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/high_level_algo_2.pdf}
   % \label{fig:high_level_algo}
\end{figure}

==> Old Makespan/makespan_programs.tex <==
In this section, we present non-convex (\NCP{}{}) and linear programming (\LP{}{}) relaxations for a given instance $(G,M,\delay)$ of DAG scheduling with fixed communication delay. We specify non-convex and linear programs in order to invoke a novel use of the ellipsoid method in Section \ref{sec:LP_solve} which allows us to find a lower bound on the optimal solution to \LP{}{} that satisfies all constraints of \NCP{}{}. We go on to prove the following two results regarding these programs. First, we show that an optimal solution to the linear program lower bounds the optimal makespan $\optmakespan$. We then show that the solution space of  \LP{}{} is a subset of the solution space of \NCP{}{}.    

The following constraints are included in both \NCP{}{} and \LP{}{}. The objective function and full constraint set of each program is given below. In the following constraints, we use $i$ to range over machines in $M$ and $u,v$ to range over jobs in $V$.

% note: should keep C > Cv as first constraint and xvi > 0 as last constraint.
\noindent
\begin{minipage}{.61\linewidth}
  \begin{flalign}
    %\min \quad \LPmakespan &
	%\tag{\ref{LP:Gen:objective}} \\
	%\text{s.t.} \quad 
	\LPmakespan &\ge \comp{v} &\forall v
	\tag{\ref{LP:Gen:makespan}}
	\\
	\start{v} &\ge \comp{u} &\forall v,u : u \prec v
	\tag{\ref{LP:Gen:predecessor}}
	\\
	\comp{v} &\ge \start{v} + \proc{v}  \sum_{i} \frac{\LPind{v}{i}}{s_i}   &\forall v
	\tag{\ref{LP:Gen:execution}}
	\\
	\start{v} &\ge \delay \sum_{j \le i} \LPind{v}{j} + S_u &\forall u,v,i: u \prec v \land \proc{u} \ge \delay\speed{i}
	\tag{\ref{LP:Gen:large_size_height}}
  \end{flalign}
\end{minipage}\hspace{6mm}%
\begin{minipage}{.34\linewidth}
  \begin{flalign}
    %\notag
    %\\
    \LPmakespan\speed{i} &\ge \sum_v \proc{v} \LPind{v}{i} &\forall i 
	\tag{\ref{LP:Gen:load}}
	\\
    \sum_i \LPind{v}{i} &\ge 1 &\forall v
	\tag{\ref{LP:Gen:cover}}
	\\
	\start{v} &\ge 0 &\forall v
	\tag{\ref{LP:Gen:nonneg_start}}
	\\
	\LPind{v}{i} &\ge 0 &\forall v,i
	\tag{\ref{LP:Gen:nonneg_indicator}}
  \end{flalign}
\end{minipage}
\vspace{4mm}

Variable $\LPind{v}{i}$ is an indicator of whether job $v$ is executed on machine $i$. Variable $\start{v}$ represents the time at which the execution of job $v$ is (first) started and variable $\comp{v}$ represents the time at which the execution of $v$ is (first) completed. Variable $\LPmakespan$ represents the makespan of the schedule. Both \NCP{}{} and \LP{}{} seek to minimize $\LPmakespan$.
Constraint~(\ref{LP:Gen:makespan}) defines the makespan as being at least as large as the last completion time.
Constraint (\ref{LP:Gen:predecessor}) ensures that a job $v$ cannot begin its execution before the completion of its predecessors. 
Constraint (\ref{LP:Gen:execution}) ensures that there is enough time between a job's start and completion times to execute the job.
Constraint~(\ref{LP:Gen:large_size_height}) ensures that a job is executed sufficiently long after  its large predecessors.
%namely that there is a $\delay$ gap between $v$'s start time and the start time of any large predecessor $u$ of $v$. 
If $v$ is executed on a machine that would take time at least $\delay$ to execute $u$, then at least $\delay$ time units must pass between the start of $u$ and the start of $v$, either for the execution of $u$ or for the communication delay.
%Intuitively, Constraint (\ref{LP:Gen:large_size_height}) uses the time needed to execute $u$ on the \textit{same machine} as $v$ to ensure that, regardless of where $u$ is actually executed, there is still a $\delay$ delay between its completion and $v$'s start times. 
Constraint~(\ref{LP:Gen:load}) ensures that the makespan is large enough that all jobs assigned to a machine can be completed.
Constraint (\ref{LP:Gen:cover}) ensures that each job is executed at least once.
%Constraints (\ref{LP:Gen:nonneg_start}) and (\ref{LP:Gen:nonneg_indicator}) ensure, respectively, that every job has non-negative start time and that every job has non-negative execution on each machine. 

We now give the final constraints that complete the specifications for the programs. 
%We refer to the non-convex and linear programs for a given instance $I$ as \NCP{}{} and \LP{}{}, respectively. 
%The subscript notation indicates that these programs have a makespan minimizing objective. This notation will distinguish the optimization programs presented here from the feasibility programs used in Section \ref{sec:LP_solve}.
\NCP{}{} and \LP{}{}  use a family of functions $\trimproc{}{i} : V \to \mathbb{Q}$ for each machine $i \in M$, defined as $ \trimproc{v}{i} = \min\{ \proc{v}, \delay\speed{i} \} $ for each $v \in V$, and $\trimsetproc{U}{i} = \sum_{u \in U} \trimproc{u}{i}$ for any set $U \subseteq V$. 
We call $\trimproc{v}{i}$ the $i$-\textit{truncated} size of job $v$.
We present the non-convex program first due to its slightly more intuitive constraint. \zoya{should probably make the order of presentation consistent between the overview and here}

The non-convex program \NCP{}{} minimizes the variable $\LPmakespan$ subject to constraints (\ref{LP:Gen:makespan}) through (\ref{LP:Gen:nonneg_indicator}) as well as the following constraint. 
\begin{align}
    \start{v} \ge \frac{\delay}{2} \sum_{j \le i}  \LPind{v}{j} + \min_{u \in A} \{ \start{u} \}  &&\forall v \in V, i \in M, A \subseteq \predex{v} : \trimsetproc{A}{i} \ge 2\delay\speed{i}
    \tag{\ref{MP:height}}
\end{align}
The following idea underlies Constraint (\ref{MP:height}). Consider a schedule in which job $v$ is executed at time $t$ on machine $j\le i$ and let $A$ be a subset of predecessors of $v$ whose total $i$-truncated size is at least $2\delay\speed{i}$. The validity of the schedule ensures that the jobs in $A$ that start their execution in the time interval $[t-\delay,t]$ are executed on $j$ and therefore have total size of at most $\delay\speed{j} \le \delay\speed{i}$. So at least half the $i$-truncated size of $A$ is made up of jobs that start before time $t-\delay$. Since the maximum $i$-truncated size of any job is $\delay\speed{i}$ there is at least one job that starts before time $t-\delay < t - \delay/2$. Note that, in principle, we could strengthen (\ref{MP:height}) to require that some job in $A$ start before time $t - \delay$. However, our algorithm requires that the feasible solution space of \NCP{}{} be a superset of the feasible solution space of \LP{}{} and the use of $\delay/2$ ensures this property holds.

The linear program \LP{}{} minimizes the variable $\LPmakespan$ subject to constraints (\ref{LP:Gen:makespan}) through (\ref{LP:Gen:nonneg_indicator}) as well as the following constraint. \zoya{should figure out if the sizes are truncated or not, and make it consistent with the previous copy of this constraint}
%$\LP{}$ has an exponential number of constraints, and we address finding a suitable solution in polynomial time in Section \ref{sec:LP_solve}. 
\begin{align}
	\start{v} &\ge \frac{\delay}{2} \sum_{j \le i} \LPind{v}{j} + \frac{\sum_{u \in A} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}} &\forall v \in V, i \in M, A \subseteq \predex{v} : \trimsetproc{A}{i} \ge 2\delay\speed{i}
	\tag{\ref{LP:Gen:height}}
\end{align}
The following idea underlies Constraint~(\ref{LP:Gen:height}).
Consider a schedule in which job $v$ is executed at time $t$ on machine $i$ and let $A$ be a set of predecessors of $v$ whose total $i$-truncated size is at least $2\delay\speed{i}$. As above, the validity of the schedule ensures that the jobs in $A$ that start in the time interval $[t-\delay,t]$ have total $i$-truncated size of at most $\delay\speed{i}$. So at least half the $i$-truncated size of $A$ is made up of jobs that start before time $t-\delay$. The family of functions $\trimproc{}{i}$ ensures that at least half the size of $A$ is made up of jobs that complete by time $t-\delay$. Constraint~(\ref{LP:Gen:height}) tells us that there is at least a $\delay/2$ gap between $t$ and the \textit{weighted average} of the completion times of all jobs in $A$.  We can view Constraint~(\ref{LP:Gen:height}) as a linear analog to the lower bound on the completion time of a job $v$ given in Definition 25 of \cite{LR02}, generalized to arbitrary speeds and job sizes.

We note that both \NCP{}{} and \LP{}{} have an exponential number of constraints and that Constraint~(\ref{LP:Gen:height}) encodes a variant of the NP-Complete knapsack problem. These considerations complicate solving the linear program and motivate our particular use of the ellipsoid method in Section \ref{sec:LP_solve}.
We proceed to verify the correctness of the \LP{}{} constraints in Lemma \ref{lem:Gen:Relaxation}.

\begin{lemma}[{\bf \LP{}{} is a valid relaxation}]
    For a given instance $(G,M,\delay)$, let $\optmakespan$ be the makespan of an optimal schedule of $(G,M,\delay)$ and let $\LPopt$ be the value of the optimal solution to \LP{}{}. Then $\LPopt \le \optmakespan$. 
\label{lem:Gen:Relaxation}
\end{lemma}

\begin{proof}
    Let $\sigma$ be a schedule of $I$ with makespan $\optmakespan$. We construct a solution to \LP{}{} with objective value $\LPmakespan \le \optmakespan$.
    
    For all $v \in V$ and $i \in M$, we set  $\comp{v}$, $\LPind{v}{i}$, and $\start{v}$ as follows. We set $\comp{v}$ to be the earliest completion time of $v$ in $\sigma$. Let $i$ be some machine on which $v$ is completed in $\sigma$ at time $\comp{v}$, choosing arbitrarily if there is more than one. Then $\LPind{v}{i} \leftarrow 1$ and $\LPind{v}{j} \leftarrow 0$ for all $j \ne i$. We set $\start{v}$ to the earliest start time of $v$ on $i$ in $\sigma$. Finally, we set $\LPmakespan \leftarrow \optmakespan$. It is easy to verify that constraints (\ref{LP:Gen:makespan}), (\ref{LP:Gen:predecessor}), (\ref{LP:Gen:execution}), (\ref{LP:Gen:cover}),  (\ref{LP:Gen:nonneg_start}), and (\ref{LP:Gen:nonneg_indicator}) are satisfied. It remains to show that (\ref{LP:Gen:large_size_height}), (\ref{LP:Gen:load}), and (\ref{LP:Gen:height}) are satisfied.
    
    We first show that constraint (\ref{LP:Gen:large_size_height}) is satisfied. As above, for any job $v$, if $\sum_{j \le i} \LPind{v}{j} = 0$, then (\ref{LP:Gen:large_size_height}) follows from (\ref{LP:Gen:predecessor}). So we fix a value of $i$ such that $\sum_{j\le i} \LPind{v}{j} = 1$. If $\predex{v} = \varnothing$ or $\proc{u} < \delay\speed{i}$ for all $u \in \predex{v}$, then there is no constraint to satisfy. So we let $u$ be some element of $\predex{v}$ such that $\proc{u} \ge \delay\speed{i}$. By the validity of $\sigma$, we know that $\start{v} \ge \comp{u}$. If $\LPind{u}{j} = 1$ for any $j \le i$, then we know that $\comp{u} - \start{u} \ge \delay$, so the constraint is satisfied. If $\LPind{u}{j} = 1$ for some $j > i$ then, by the fact that $\sigma$ satisfies the communication delay $\delay$, we have that $\start{v} \ge \comp{u} + \delay \ge \start{u} + \delay$, from which (\ref{LP:Gen:large_size_height}) follows.

    We now show that constraint (\ref{LP:Gen:load}) is satisfied. For any machine $i$, let $W_i$ be the set of all jobs $v$ such that some copy of $v$ is executed on $i$ in $\sigma$, i.e. $W_i$ is the amount of work done on machine $i$. Since our variable assignment ignores all but the earliest completed copy of $v$, we have that
    $\LPmakespan \speed{i} = \optmakespan \speed{i} \ge \setproc{W_i} \ge \sum_v \proc{v} \LPind{v}{i}$,
    from which (\ref{LP:Gen:load}) follows.
    
    Finally, we show that constraint (\ref{LP:Gen:height}) is satisfied. Since we have $\LPind{v}{i} = 1$ for exactly one machine $i$, for any $j$ we have that $\sum_{j' \le j} \LPind{v}{j'} = 1$ or $\sum_{j' \le j} \LPind{v}{j'} = 0$. Suppose $\sum_{j \le i} \LPind{v}{j} = 0$ and let $A \subseteq \predex{v}$ be such that $\trimsetproc{A}{i} \ge 2\delay\speed{i}$. By constraint (\ref{LP:Gen:predecessor}), we have that $\comp{u} \le \start{v}$ for all $u \in A$. So 
    \[ \start{v} = \start{v} \cdot \frac{\trimsetproc{A}{i}}{\trimsetproc{A}{i}} \ge \frac{\delay}{2} \sum_{j \le i} \LPind{v}{j} + \frac{\sum_{u \in A} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}}.\]
    So we fix the value of $i$ such that $\sum_{j' \le i} \LPind{v}{j'} = 1$. This entails that the earliest completion of $v$ was on some machine $j \le i$. We also fix this value of $j$. Recall that this implies $\speed{j} \le \speed{i}$.

    We now establish that (\ref{LP:Gen:height}) is satisfied in the case that $\sum_{j' \le i} \LPind{v}{j'} =1$. Let $A \subseteq \predex{v}$ be such that $\trimsetproc{A}{i} \ge 2\delay\speed{i}$. We divide this analysis into two cases. We call job $u \in A$ a \textit{threshold job} of $v$ if $\start{u} < \start{v} - \delay < \comp{u}$. In the first case, we suppose there is no threshold job of $v$. Then, for all $u \in A$, we have that either $\start{u} \ge \start{v} - \delay$ or $\comp{u} \le \start{v}-\delay$. Let $A' = \{ u : \comp{u} \le \start{v} - \delay \} \cap A$ be the set of jobs in $A$ that complete before time $\start{v} - \delay$. In this case, all jobs in $A \setminus A'$ start and complete on machine $i$ in the time interval $[\start{v} - \delay, \start{v}]$. So, we have that $\trimsetproc{A \setminus A'}{i} \le \delay\speed{i} \le \trimsetproc{A}{i}/2$. So
    \begin{align*}
        \frac{\sum_{u \in A} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}} &= \frac{\sum_{u \in A \setminus A'} \trimproc{u}{i} \comp{u} + \sum_{u \in A'} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}} 
        \\
        &\le \frac{\start{v} \sum_{u \in A \setminus A'} \trimproc{u}{i} + (\start{v} - \delay) \sum_{u \in A'} \trimproc{u}{i} }{\trimsetproc{A}{i}} &\text{by definition of}~ A ~\text{and}~ A'
        \\
        &= \start{v} - \frac{\delay \sum_{u \in A'} \trimproc{u}{i}}{\trimsetproc{A}{i}} \le  \start{v} - \frac{\delay}{2}
    \end{align*}
    where the final inequality follows from $\trimsetproc{A'}{i} \ge \trimsetproc{A}{i}/2$.
    %\[ \frac{\sum_{u \in A} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}} \le \frac{\sum_{u \in A \setminus A'} \trimproc{u}{i} \comp{u} + \sum_{u \in A'} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}} \le \frac{\start{v} \sum_{u \in A \setminus A'} \trimproc{u}{i} + (\start{v} - \delay) \sum_{u \in A'} \trimproc{u}{i} }{\trimsetproc{A}{i}} \le \start{v} - \frac{\delay}{2}. \]
    
    We now show that (\ref{LP:Gen:height}) is satisfied for the second case in which $\sum_{j'\le i} \LPind{v}{j'} = 1$ and there is some threshold job $\theta$ of $v$. By definition of $\theta$ and the validity of $\sigma$, we have that $\theta$ is the only threshold job of $v$ and $\LPind{\theta}{j} = 1$. We let $X = \speed{i}(\start{v} - \comp{\theta})$ and let  $Y = \trimproc{\theta}{i}$. We define $A'$, as above, to be the subset of jobs $u \in A$ such that $\comp{v} \le \start{v} - \delay$. Figure \ref{fig:height_validity} illustrates the definitions of $A'$ and the threshold job $\theta$. Then we have
    \begin{align*}
        \frac{\sum_{u \in A} \trimproc{u}{i} \comp{u}}{\trimsetproc{A}{i}} &\le \frac{\start{v} \trimsetproc{(A \setminus A') \setminus \{\theta\}}{i} + \comp{\theta} \trimproc{\theta}{i} + (\start{v} - \delay)  \trimsetproc{A'}{i}}{\trimsetproc{A}{i}} &\text{by definition of}~ A' ~\text{and}~ \theta
        \\
        &\le \frac{\start{v}X + (\start{v} - \frac{X}{\speed{i}}) Y + (\start{v} - \delay)\trimsetproc{A'}{i}}{\trimsetproc{A}{i}} &\text{by definition of}~ X ~\text{and}~ Y
        \\
        &= \frac{\start{v}X + \start{v}Y + \start{v}\trimsetproc{A'}{i} - \frac{X}{\speed{i}}Y - \delay \trimsetproc{A'}{i}}{\trimsetproc{A}{i}} &\text{by calculation}
        \\
        &\le \start{v} - \delay \bigg( \frac{\trimsetproc{A}{i} - X - Y + \frac{XY}{\delay\speed{i}}}{\trimsetproc{A}{i}} \bigg) &\text{by}~ \trimsetproc{A}{i} = X + Y + \trimsetproc{A'}{i}
        \\
        &= \start{v} - \delay + \delay \bigg( \frac{ X + Y - \frac{XY}{\delay\speed{i}} }{\trimsetproc{A}{i}} \bigg)  &\text{by calculation}
        \\
        &\le \start{v} - \delay + \delay \bigg( \frac{ X + Y - \frac{XY}{\delay\speed{i}} }{2\delay\speed{i}} \bigg)  &\text{by}~ \trimsetproc{A}{i} \ge 2\delay\speed{i}.
    \end{align*}
    So we must show only that $X + Y - \frac{XY}{\delay\speed{i}} \le \delay\speed{i}$. By definition of $X$ and $Y$, we have that $X + Y \ge \delay \speed{i}$ and $X \le \delay\speed{i}$ and $Y \le \delay\speed{i}$. We fix the value of $X + Y$ to be $\alpha$. In this case, $XY$ is minimized when $X = \delay\speed{i}$ and $Y = \alpha - \delay\speed{i}$. So $ X + Y - \frac{XY}{\delay\speed{i}} \ge \alpha - \frac{\delay\speed{i}(\alpha - \delay\speed{i})}{\delay\speed{i}} = \delay\speed{i} $  from which (\ref{LP:Gen:height}) follows.
    \begin{figure}
        \centering
        \includegraphics{Figures/height_constraint_validity.pdf}
        \caption{All jobs are represented by boxes, with time increasing from left to right. Machine indices are shown on the left and are increasing from top to bottom. The job $v$ and its threshold job $\theta$ are labeled. Other than $v$, all jobs depicted are elements of $A \subseteq \predex{v}$. The set $A'$ is shown in gray.}
        \label{fig:height_validity}
    \end{figure}
\end{proof}

Finally, we show that the feasible solution space of \NCP{}{} is a superset of the feasible solution space of \LP{}{}. This will be essential for our use of the ellipsoid method in Section \ref{sec:LP_solve}.


\begin{lemma}[{\bf \NCP{}{} is a subset of \LP{}{}}]
    Any assignment of values to all variables $\LPind{v}{i}$, $\start{v}$, $\comp{v}$, and $\LPmakespan$ that satisfies \LP{}{} also satisfies \NCP{}{}.
    \label{lem:LP_subset_MP}
\end{lemma}

\begin{proof}
    For a given variable assignment, suppose that constraint (\ref{MP:height}) of \NCP{}{} is violated for some choice of $i \in M$, $v \in V$, and $A \subseteq \predex{v}$, which means that for all $u\in A$,  $\start{u} \ge \start{v} - \frac{\delay}{2} \sum_{j \le i} \LPind{v}{j}$. Then $\trimsetproc{A}{i} \ge 2\delay\speed{i}$.
    So
    \begin{align*}
        \frac{\sum_{u \in A}\trimproc{u}{i}\comp{u}}{\trimsetproc{A}{i}} &> \frac{\sum_{u \in A}\trimproc{u}{i}\start{u}}{\trimsetproc{A}{i}} &\text{by Constraint (\ref{LP:Gen:execution})}
        \\
        & \ge 
        \frac{(\start{v} - \frac{\delay}{2}\sum_{j \le i} \LPind{v}{j}) \trimsetproc{A}{i}}{\trimsetproc{A}{i}} &\text{by supposition}
        \\
        &= \start{v} - \frac{\delay}{2} \sum_{j \le i} \LPind{v}{j}.
    \end{align*}
    Therefore, Constraint (\ref{LP:Gen:height}) is also violated.
\end{proof}

==> Old Makespan/preprocess.tex <==
In this section, we present the first subroutine of our algorithm. Given an instance $I = (G,M,\delay)$, this subroutine outputs a new instance $I' = (G, M', \delay)$ such that $M' \subseteq M$ such that the speed of each machines in $M'$ is within a factor of $m$ of the speed of the fastest machine in $M$. More formally, 
\[ M' = \{ i \in M : \speed{i} \ge \speed{m}/m\}  \]
where machine $m$ is the fastest machine in $M$. The following lemma is proved in Appendix \ref{sec:elim_slow_machines}.

\begin{lemma}
    Let $\optmakespan$ be the optimal makespan on instance $I$ and $C'$ be the optimal makespan on $I'$. Then $C' \le 6 \optmakespan$.
    \label{lem:elim_slow}
\end{lemma}

The proof in Appendix~\ref{sec:elim_slow_machines} shows that, any schedule $\sigma_1$ on $I = (G,M,\delay)$ with makespan $C_1$ can be converted into a schedule $\sigma_2$ on $I$ with makespan $C_2 \le 6 C_1$ where the speeds of all machines used in $\sigma_2$ are within a factor of $m$ of the fastest machine in $M$.
We note that an alternative strategy for eliminating these machines is given in \cite{chudak1999approximation}. There, the authors argue that any solution to their linear program on $I$ can be converted into a solution to their linear program on $I'$. A corresponding result can be proved for either our linear or non-convex programs.  We choose to use the method given in Appendix \ref{sec:elim_slow_machines} because the bound proved there holds for the optimal \textit{makespan} of $I$, rather than the optimal program solution on $I$. This means that the result holds regardless of which program formulation is used and, therefore, has greater independent interest. 

==> Old Makespan/solveNCP.tex <==
In this section, we present the second subroutine which finds a feasible solution to \NCP{}{} that lower bounds the optimal solution to \LP{}{}, for a given instance $(G,M,\delay)$ of DAG scheduling with fixed communication delay.
The subroutine uses the ellipsoid method of \cite{KHACHIYAN198053, schrijver:3572397410982} to handle the exponential number of constraints given by (\ref{LP:Gen:height}).
However, because constraint (\ref{LP:Gen:height}) encodes an NP-Complete problem (a variant of knapsack) we do not know of an exact polynomial time separation oracle for \LP{}{}. We overcome this obstacle by a novel use of the ellipsoid method that may be of independent interest.

In order to invoke the ellipsoid method, we convert our optimization problem into a feasibility problem. We define the linear feasibility program \LP{}{\guess} as the set of constraints (\ref{LP:Gen:makespan}) through (\ref{LP:Gen:nonneg_indicator}),  constraint (\ref{LP:Gen:height}), and the following constraint.
\begin{align}
    C \le \guess 
    \label{LP:guess}
\end{align}
where $\guess$ is some guessed makespan. 
Similarly, we define the non-convex feasibility program \NCP{}{\guess} as the set of constraints (2) through (9) along with constraints (\ref{MP:height}) and (\ref{LP:guess}). 
\junk{
\begin{align}
    \min_{u \in A} \{ \start{u} \} \le \start{v} - \frac{\delay}{2} \sum_{j \le i} \LPind{v}{j} &&\text{for all}~ v \in V, i \in M, \text{and}~ A \subseteq \predex{v} ~\text{s.t.}~ \trimsetproc{A}{i} \ge 2\delay\speed{i}
    \tag{\ref{LP:Gen:height}\textsuperscript{+}}
    \label{MP:height}
\end{align}
}
%For given $\guess$ and $\instance$, we define $\LPspace$ and $\MPspace$ to be the solution spaces of \LP{}{\guess} and \NCP{}{\guess}, respectively.
Throughout the section, we use $\vector{x}$ to be an assignment of to all variables $\{\LPind{v}{i},S_v,C_v\}_{v,i}$. We say that an assignment $\vector{x}$ is \LP{}{\guess}-feasible \NCP{}{}-feasible if $\vector{x}$ satisfies all constraints of \LP{}{\guess} or \NCP{}{\guess}, respectively. Similarly, we say $\vector{x}$ is \LP{}{\guess}-infeasible or \NCP{}{\guess}-infeasible if it fails to satisfy any constraints of the respective programs.
Our use of the ellipsoid method combines the results of the following lemma to either find a feasible solution to \NCP{}{\guess} or determine that there is no feasible solution to \LP{}{\guess}.

\begin{lemma}[{\bf \NCP{}{} Membership and \LP{}{} separation}]
    There is a polynomial time membership oracle \oracle{} for \NCP{}{\guess}. Also every \LP{}{\guess}-feasible $\vector{x}$ is \NCP{}{\guess}-feasible and, for any \NCP{}{\guess}-infeasible $\vector{x}$, there is a polynomial time computable hyperplane separating $\vector{x}$ from the set of \LP{}{\guess}-feasible variable assignments. 
    \label{lem:MP_membership}
\end{lemma}

\begin{proof}
    We first prove the existence of \oracle{} for \NCP{}{\guess}. Given any assignment $y$ of values to all variables $\LPind{v}{i}, \start{v}, \comp{v}$, and $\LPmakespan$ of \NCP{}{\guess}, we can easily check all constraints other than (\ref{MP:height}) in polynomial time. To verify  (\ref{MP:height}) for any $v \in V$ and $i \in M$, we construct the set $A = \{ u \in \predex{v}: \start{u} > \start{v} - \frac{\delay}{2}\sum_{j \le i} \LPind{v}{j}\}$. If $\trimsetproc{A}{i} \ge 2 \delay\speed{i}$, then constraint (\ref{MP:height}) is violated for these $v$, $i$, and $A$. If any constraints are violated the oracle returns that $y$ is infeasible for \NCP{}{\guess}. Otherwise, the oracle returns that $y$ is feasible for \NCP{}{\guess}.
        
    By Lemma~\ref{lem:LP_subset_MP}, we have that all solutions to \LP{}{\guess} are feasible for \NCP{}{\guess}. So, for any $y$ infeasible for \NCP{}{\guess} we have that $y$ violates some constraint of \LP{}{\guess} which gives a separating hyperplane. By the existence of \oracle{} and the proof of Lemma~\ref{lem:LP_subset_MP}, we have that this violated constraint of \LP{}{\guess} is polynomial time computable. 
\end{proof}

\begin{lemma}[{\bf Solving \NCP{}{\guess} when  \LP{}{\guess} is feasible}]
    There is a polynomial time algorithm that takes as input $\guess$ and either returns a feasible solution to \NCP{}{\guess} or correctly determines that \LP{}{\guess} is infeasible.
    \label{lem:nonemptiness}
\end{lemma}

Our proof of Lemma \ref{lem:nonemptiness} relies on the following lemma, which we restate here for completeness.

\begin{lemma}
    [{\bf Theorem 6.4.1 in \cite{schrijver:3572397410982}}]
    The strong nonemptiness problem for well-described polyhedra given by a strong separation oracle can be solved in oracle-polynomial time.
    \label{lem:schriver_nonemptiness}
\end{lemma}

The strong nonemptiness problem is defined as follows: given compact and convex space $\mathcal{S}_0$, find a point in $\mathcal{S}_0$ or determine that $\mathcal{S}_0$ is empty (see Section 2.1 in \cite{schrijver:3572397410982}). 
A polyhedron is ``well-described'' if all faces can be given by inequalities of constant length (definition (6.2.2) in \cite{schrijver:3572397410982}). Since the solution space of \LP{}{\guess} is well-described, it remains only to show that it is given by a strong separation oracle. Toward this end, we define Algorithm \ref{alg:separation_oracle}.

\begin{algorithm}
    \KwData{an assignment $\vector{x}$ of values to all variables $\LPind{v}{i}, \start{v}, \comp{v}$, and $\LPmakespan$}
    \KwResult{indication that $\vector{x}$ is \NCP{}{\guess}-feasible or a hyperplane separating $\vector{x}$ from \LP{}{\guess}-feasible assignments}
    run \oracle{} on $\vector{x}$\;
    \uIf{\oracle{} returns that any constraint (\ref{LP:Gen:makespan}) through (\ref{LP:Gen:nonneg_indicator}) or (\ref{LP:guess}) is violated}{
        \Return the violated constraint\;
    }
    \uElseIf{\oracle{} returns that constraint (\ref{MP:height}) is violated on $v \in V$, $i \in M$, and set $A$}{
        \Return constraint (\ref{LP:Gen:height}) violated on $v$, $i$, and $A$\;
    }
    \Else{ \Return $\vector{x}$ is \NCP{}{\guess}-feasible\; }
    \caption{Relaxed Separation Oracle for \NCP{}{\guess}}
    \label{alg:separation_oracle}
\end{algorithm}

\begin{proof}
    [Proof of Lemma \ref{lem:nonemptiness}]
    To meet the conditions of Lemma \ref{lem:schriver_nonemptiness}, we define a strong separation oracle \oracle{\LP{}{}} for \LP{}{\guess}. Given a point $\vector{x}$, \oracle{\LP{}{}} runs \oracle{} on $\vector{x}$. If \oracle{} returns a violated constraint, then \oracle{\LP{}{}} returns the same violated constraint. If \oracle{} returns that $\vector{x}$ is \NCP{}{\guess}-feasible then \oracle{\LP{}{}} checks if $\vector{x}$ satisfies constraint (\ref{LP:Gen:height}). If not, \oracle{\LP{}{}} returns the violated constraint. Otherwise, \oracle{\LP{}{}} returns that $y$ is \LP{}{\guess}-feasible.
    
    We show that \oracle{\LP{}{}} is a strong separation oracle for \LP{}{\guess}. By definition (2.1.4) in \cite{schrijver:3572397410982}, a strong separation oracle either indicates that a given point $\vector{x}$ is \LP{}{\guess}-feasible or gives a hyperplane separating $\vector{x}$ from the set of \LP{}{\guess}-feasible assignments. The oracle \oracle{\LP{}{}} satisfies this definition by Lemma \ref{lem:MP_membership}.
    So, by Lemma \ref{lem:schriver_nonemptiness}, the strong nonemptiness problem for \LP{}{\guess} is solved in oracle-polynomial time with oracle \oracle{\LP{}{}}.
    
    Suppose we run the ellipsoid algorithm using Algorithm~\ref{alg:separation_oracle} as the separation oracle, and suppose that in the course of running the ellipsoid algorithm there are $d$ calls made to Algorithm~\ref{alg:separation_oracle}.
    Then the ellipsoid method with \oracle{\LP{}{}} makes at least $d$ calls to \oracle{\LP{}{}}: for a given assignment $\vector{x}$, \oracle{\LP{}{}} may return a violated constraint (\ref{LP:Gen:height}) where Algorithm~\ref{alg:separation_oracle} returns that $\vector{x}$ is \NCP{}{\guess}-feasible. Therefore, the ellipsoid method using Algorithm \ref{alg:separation_oracle} runs in oracle polynomial time. The lemma follows from the fact that
    %Algorithm~\ref{alg:separation_oracle}
    \oracle{} is a polynomial time membership oracle per Lemma~\ref{lem:MP_membership}.
\end{proof}

\begin{lemma}[{\bf Solving \NCP{}{}}]
    In polynomial time, we can find a feasible solution to \NCP{}{\optmakespan}, where $\optmakespan$ is the optimal makespan of the given isntance.
    \label{lem:MP_solution}
\end{lemma}

\begin{proof}
    Let $\LPopt$ be the optimal solution to \LP{}{}. 
    We show that the number of iterations of the ellipsoid method needed to find $\LPopt$ is polynomial in the length of the input $I$.
    By Lemma~\ref{lem:Gen:Relaxation}, we have that $\LPopt \le \optmakespan$, where $\optmakespan$ is the optimal makespan on $I$. Further, we can upper bound $\optmakespan$ by the amount of time needed to run all jobs on the fastest machine, i.e.\ $\optmakespan \le \setproc{V}/\speed{m}$. So, $0 \le \LPopt \le \setproc{V}/\speed{m}$. Our algorithm searches the space of \textit{good} schedules, where a schedule is good if, given an ordering of job start times on each machine, all jobs are executed as early as possible given the constraints of the problem, in particular the precedence and communication delay constraints. Clearly the optimal schedule is a good schedule.
    
    We show that if the difference in the makespans of two good schedules is $\delta$ then the length of $\delta$ is polynomial in the length of $I$. Let  $\sigma$ be an arbitrary schedule with makespan $C$. We construct a chain $\chain$ of job-machine pairs $\link{1}, \ldots, \link{|\chain|}$ recursively as follows. Let 
    \begin{align*}
        \link{|\chain|} &= \argmax_{(v,i) \in V \times M}\{ \sigma[v,i] + \proc{v}/\speed{i}  : \sigma[v,i] \ne \bot \} \quad \text{and}
        \\
        \link{x-1} &= \argmax_{(v,i) \in V \times M} \Big\{ \{ \sigma[v,i] + \proc{v}/\speed{i}  : \link{x} = (u,i) ~\text{and}~ \sigma[v,i] \ne \bot ~\text{and}~ \sigma[v,i] < \sigma[u,i] \},
        \\
        &\hspace{24mm} \{ \sigma[v,i] + \proc{v}/\speed{i}: \link{x} = (u,j) ~\text{and}~ \sigma[v,i] \ne \bot ~\text{and}~ v \in \predex{u}\} \Big\}.
    \end{align*}
    Intuitively, we can think of the chain as stepping backward through the schedule $\sigma$. The first link $\link{|\chain|}$ is the last job-machine pair to complete in $\sigma$. Then, for any given link $(v,i)$, the previous link is the job-machine pair $(u,j)$ such that either $u$ is a predecessor of $v$ or $i=j$ and $(u,i)$ completes before $(v,i)$, depending on which has larger completion time. 
    By construction and the fact that $\sigma$ is a good schedule, the first job in the chain starts at time 0 and the last completes at time $C$. So, $C$ can be represented as $b\delay + \sum_{(v,i) \in \chain} \proc{v}/\speed{i}$ for some integer $b$.
    
    We now consider two good schedules, $\sigma_1$ and $\sigma_2$ with respective makespans $C_1$ and $C_2$ such that $C_1 > C_2$. Since both $C_1$ and $C_2$ can be represented in the form $b\delay + \sum_{(v,i) \in \chain} \proc{v}/\speed{i}$, their difference is at least $1/(d\prod_{i \in M} \speed{i})$, where $\delay$ is some rational number $c/d$. So, the length of $\delta$ is polynomial in the length of the instance $I$. Therefore, the number of necessary calls to the ellipsoid method is also polynomial in the length of $I$. 
\end{proof}

==> Special_Case_Bounds.tex <==
\section{Better Bounds for Special Cases}
\label{sec:special_case_bounds}

\zoya{Check if these are the correct proofs and move them into the paper body}

\begin{proof}
    [Proof of Claim \ref{claim:load_phases}]
    Since all jobs take at least $2\rho$ time on all machines, then in each band all jobs are independent by lemma \ref{lem:Gen:HeightBound}. So, there can be only $O(1)$ height phases of $\phasetype{\tau}$ per band. This removes the $\log(\rho m)$ numerator term in our approximation ratio. Since the other terms do not rely on machine speeds, we can scale everything so that $\rho=1$, which gives the desired bound. 
\end{proof}

\begin{proof}
    [Proof of Claim \ref{claim:finishing_phases}]
    This result requires changing the algorithm to have an overlap parameter $(1 - 1/\gamma)$ rather than using 1/2. The idea is that, if there is only one speed, we can eliminate all talk of median machines, and get an approximation ratio of $O(\gamma + \log_{\gamma}\rho)$. Setting $\gamma$ to $\log\log\rho/\log\rho$ gives the desired bound.
    
    \david{possibly also relies on the algo operating over speeds instead of machines}
\end{proof}

==> ToDo.tex <==
\begin{itemize}
    \item Editing improvements to STOC paper
    \begin{itemize}
        \item write theorem in terms of number of groups - not $\log m$ - in order to address the fact that we get a better approximation with unit speed
        \item talk about linear delay constraints only in the section on solving NCP - we don't need to refer to it outside this context. this would mean we don't have to explain truncated size in our intro
        \item in intro - motivate our method using unit speed / capacity? can prove that num of ancestors in a band is $O(\delay)$ and then argue that a band can be completed in $\log \delay$ phases. could even 
        \item discuss why the generalized Kulkarni et al LP fails in related work
        \item present each subroutine as an isolated algorithm with input and output. 
        \item separate analysis into a new subsection where we reason over the performance of the algorithm as a whole.
        \item sell paper as solving both duplication and non-duplication problems
        \item knapsack cover inequalities to solve NCP
        \item is there an more generally applicable algorithmic take-away?
        \item discuss alternative LP formulations and why we don't use them (in separate appendix)
        \begin{itemize}
            \item time-indexed LP from Kulkarni et al
            \item time-indexed version of our LP
        \end{itemize}
        \item give examples of duplication being used in industry
        %\item add section on efficiency of makespan algorithm \zoya{what do you mean?}
    \end{itemize}
    
    \item short term technical questions
    \begin{itemize}
        \item Kulkarni et al allow that communication delays are variable, but upper bounded by a constant. Can we make a similar assumption?
        \item can we simplify the conversion from LP solution to the schedule?
        \item algorithm for minimizing average completion time
        \item reduce makespan approximation by factor of $\log\log m$
        \item find example where minimum makespan without duplication is a $\log n$ factor higher than the minimum makespan with duplication
        \item reduce $\log^3$ factor in no-duplication upper bound
        \item write up non-convex solver as a general method and just apply it in our case
    \end{itemize}
    
    \item Long term questions
    \begin{itemize}
        \item general communication delays
        \item hierarchical communication delays
        \item hardness for completing schedule in one phase
        \item generalizing integrality gap
        \item eliminate reliance on ellipsoid method to reduce runtime
        \item reformulating algorithm to work in a different setting: distributed, online, etc.
    \end{itemize}
\end{itemize}

==> arxiv_abstract.tex <==
We consider the problem of scheduling $n$ precedence-constrained jobs on $m$ uniformly-related machines in the presence of an arbitrary, fixed communication delay $\rho$. We consider a model that allows job duplication, i.e. processing of the same job on multiple machines, which, as we show, can reduce the length of a schedule (i.e., its makespan) by a logarithmic factor. Our main result is an $O(\log m \log \rho / \log \log \rho)$-approximation algorithm for minimizing makespan, assuming the minimum makespan is at least $\rho$. Our algorithm is based on rounding a linear programming relaxation for the problem, which includes carefully designed constraints capturing the interaction among communication delay, precedence requirements, varying speeds, and job duplication. Our result builds on two previous lines of work, one with communication delay but identical machines (Lepere and Rapine 2002) and the other with uniformly-related machines but no communication delay (Chudak and Shmoys 1999).

We next show that the integrality gap of our mathematical program is $\Omega(\sqrt{\log \rho})$.  Our gap construction employs expander graphs and exploits a property of robust expansion and its generalization to paths of longer length. Finally, we quantify the advantage of duplication in scheduling with communication delay.  We show that the best schedule without duplication can have makespan $\Omega(\rho/\log \rho)$ or $\Omega(\log m/\log\log m)$ or $\Omega(\log n/\log \log n)$ times that of an optimal schedule allowing duplication.  Nevertheless, we present a polynomial time algorithm to transform any schedule to a schedule without duplication at the cost of a $O(\log^2 n \log m)$ factor increase in makespan.  Together with our makespan approximation algorithm for schedules allowing duplication, this also yields a polylogarithmic-approximation algorithm for  the setting where duplication is not allowed.  

==> reviews.tex <==
Review \#865A
===============

Paper summary
-------------
The paper considers the problem of scheduling jobs on related machines (each machine has a speed and processing time of a job $j$ on machine $i$ is volume of $j$ divided by speed of $i$) under job precedence constraints and communication delays. Before we can begin a job $j$ all preceding jobs should have completed. Further, if job $j$ is scheduled on machine $i$ and a preceding job $j'$ on machine $i'$ then there should be a gap of at least $\rho$ between the completion time of $j'$ and the start of job $j$; this is due to the delay in communicating results from one machine to another.

In the absence of communication delays an $O(\log m)$ approximation is known for the problem of minimizing makespan. This paper gives the first result which makes no assumptions on numbers of machines, size of jobs or communication delay and gives a polylog approximation. An interesting aspect of the results is that it uses the fact that duplicating jobs in presence of communication delays can reduce total makespan. The paper also shows that removing job duplication only incurs an additional polylog overhead in the makespan.

The authors formulate this problem as a non-convex program (NCP) and as a linear program with exponentially many constraints. They then employ a  procedure to solve the NCP which uses the ellipsoid method and seems to go between the NCP and the LP. I have not seen anything like this before and am not convinced of the merit of this. \hl{I suggest that the authors check alternate ways to formulate the LP which would make it efficiently solvable. In particular an easy way to capture communication delays would have been: if $u$ precedes $v$ then $S_v-C_u \ge \rho(1-*\sum_i\delta_{i,u,v})$ where $\delta_{i,u,v}\le x_{v,i}$ and $\delta_{i,u,v}\le x_{u,i}$. Note here $\rho\delta_{i,u,v}$ is the savings in communication delay due to $u,v$ being scheduled on machine $i$.}

Post the solution to the NCP/LP the authors divide machines into $\log m$ groups and assign jobs to groups. This is standard and has been used in previous work. Converting the assignment into a schedule also seems tricky in this setting and the authors \hl{have a set of 4 rules to determine when a job is scheduled on a machine. I did not find this very intuitive or elegant.}

Overall, I feel that although the paper makes progress on an interesting problem, \hl{there isn't a sufficiently insightful contribution in terms of the approach and the algorithm.}


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review \#865B
=================

Paper summary
-------------
Summary:

This paper studies the problem of scheduling n precedence-constrained jobs on m uniformly-related machines when jobs have a fixed communication delay rho. There are n jobs with precedence constraints given by a DAG G, and m machines. Each job v has a size $p_v$, each machine i has a speed $s_i$ and the processing time of v on i is $p_v/s_i$. When a job u precedes v in G, then v can only start after u completes if they are scheduled on the same machine, and rho units time after u completes when they are scheduled on different machines. In the problem, jobs must be non-preemptively scheduled, but duplication of jobs is allowed: copies of a job v can be scheduled on different machines; this may help in reducing the communication cost.  The goal of the problem is to schedule all the jobs so as to minimize the makespan of the schedule.

The main result of the paper is an O(log m * log rho / log log rho)-approximation for the problem when we have OPT $\ge$ rho.  The algorithm is based on a novel non-convex program (NCP) for the problem and a rounding procedure that combines two previous ones: the one by Lepere and Rapine for the same problem but on identical machines, and the other one by Chudak and Shmoys for the problem without communication cost.  I now describe the two components one by one.

Other than polynomial number of natural linear constraints, the NCP contains a non-convex constraint ((1) in the paper). The NCP can not be solved directly, and the authors formulated an linear program (LP) with exponential number of constraints. The LP polytope is shown to be contained in the NCP feasible region (i.e, LP $\subseteq$ NCP).  However, the LP could not be solved efficiently as it involves the NP-hard knapsack problem. Given a solution x, the authors gave a procedure that does the following: either claims that x $\in$ NCP, or finds a constraint that separates x from LP.  Using the ellipsoid method, one can find in polynomial time a x $\in$ NCP.

The second component is the rounding algorithm. As in Chudak and Shmoys (and a recent paper of Li), the algorithm breaks the machines into $\log_2 m$ groups, each containing machines with speeds differing by a factor of at most 2 (by standard techniques, one can assume the maximum and minimum speeds differ by at most a factor of m). Then each job v is assigned to one group according to the LP solution (or NCP solution). Roughly speaking, v is assigned to a not-too-slow group with the largest capacity (the capacity of a group is the total speed of machines in the group).  This guarantees that (1) the processing time of a job v, when assigned to a machine in its assigned group, is not too big compared to the LP solution, and (2) the total load of all groups is small compared to the LP solution.  With the two conditions, a simple list scheduling algorithm respecting the assignment can give the result of Chudak and Shmoys for the problem without communication delay.

To extend the rounding algorithm to the communication delay setting, the authors designed the list-scheduling algorithm more carefully. In particular, it uses some ideas from the result of Lepere and Rapine for the communication delay problem in the identical-machine setting.  The algorithm proceeds in phases of length 5 rho. In each phase, it considers the groups and the jobs in some order. It schedules a job and its predecessor on a machine in the group if it satisfies some conditions (C1 - C5 in the paper), which combines the ideas from Chudak and Shmoys and Lepere and Rapine. In the analysis, the authors show that in each phase, the algorithm is making some progress so that the makespan will be bounded in terms of the LP solution.

Strength and Weakness:

In general, scheduling problems in the presence of communication delay are very hard. There were only a few previous results for this model, but in much simpler settings than the one considered in this paper. Many of them need to assume that the machines are identical, m = O(1), $\rho = O(1)$ and/or the job sizes are the same.  This paper is the first one to give an approximation algorithm with small approximation gurantee for the related machine scheduling model in the presence of an arbitrarily large communication delay rho.  In terms of the techniques, the paper combine ingredients from the two previous results mentioned above, but the formulation of the non-convex program is interesting, and the design and analysis of the rounding algorithm are highly non-trivial.  They may give insights into some more general settings such as arbitrary delay function and the unrelated machine environment.  Overall, I think the paper should be accepted to STOC.

Targeted Audience: algorithm design researchers

Comments for authors
--------------------
A major comment:

\hl{The framework for solving the NCP has been used before, for example, for the knapsack covering problem by Carr et al, (they derived the knapsack covering inequalities) and the capacitated facility location problem by An et al.}  In these results, the formulated LP contains exponential number of constraints and can not be solved efficiently. However only a small number of the constraints matter (the constraints depend on the fractional solution and thus can not be determined at the beginning).  Then given a solution, one can efficiently check if the critical constraints are satisfied or not. Using the ellipsoid method, one can find a solution which satisfies these critical constraints.   \hl{It might be better if the authors describe their LP and NCP using this framework.  In particular, I think it is cleaner to use the following order: first describe the LP, then show the critical constraints in the LP, and finally show that if the constraints are satisfied, then the constraint (1) (i.e, the non-convex constraint) is satisfied.  In the current writeup, the critical constraints are implicitly used in the proof of Lemma 4.2. Then in the proof of Lemma 4.4, the authors say that a violating LP constraint can be found efficiently using the proof of Lemma 4.2. I feel that this is not the perfect way to make the proof.}

More crucially, \hl{I am wondering if the LP constraint (2) is captured using the Knapsack Covering inequalities introduced by Carr et al.}

\hl{Minor comments:}

-Second paragraph of Page 12: change "use use" to "use"
-First paragraph of Page 16: The NCP contains constraints (3) through (10) (instead of (2) through (9))?
-Page 20, the paragraph starting with ``First (C1)'': at least rho time phase tau $\ge$ at least rho time *in* phase tau.
-page 21, Algorithm 2, Line 14.  The phrase for all $v \in V \setminus$ (Current $\cup$ Completed) is a bit confusing since Current and Completed might change in the loop.  Does it mean (i) that for all $v \in V \setminus$ (Current $\cup$ Completed) for the (Current $\cup$ Completed) at the beginning of the for loop, or (ii) that we repeat the procedure until all $v \in V \setminus$ (Current $\cup$ Completed) have been considered, where we the sets Current and Complete as dynamic sets?


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review \#865C
=======================

Paper summary
-------------
This paper considers a rather baroque variant of several well-studied scheduling problems - minimizing makespan on machines that run uniformly at different speeds subject to precedence constraints but where there is a communication delay associated with each precedence relation if the related jobs are assigned to different machines (and since there is an advantage to having job processed on the same machine as its predecessor, there is an advantage to job duplication.

At a high level, the main structural approach follows the broad outlines of its predecessors - one of the quirks of the scheduling literature is that the variant without communication delays is one of the few settings where a constant approximation might be possible, and yet the best algorithms have performance guarantee O(log m), where m is the number of machines.

The technical challenges in accommodating the communication delays seem to be formidable, and the interplay between the LP relaxation and the non-convex relaxation (which is new to this paper) is an ingenious way to make progress. However, the complexity in doing so leaves this reader with the feeling that while this technical progress has been carefully engineered to work in this setting, \hl{it does not feel like there is a new to-be-used-regularly tool that has been added to the algorithmic toolkit.}


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review \#865D
=================

Paper summary
-------------
The paper studies scheduling jobs on related machines (machines have different speeds) under precedence constraints and uniform communication delays and duplication allowed. Main result is a poly-log approximation under a natural condition on the delay parameter.

The paper uses several tools in scheduling and approximation I won't summarize the details here.
However, I do not believe the paper is a good fit for STOC for several reasons that I list below.

- \hl{The paper assumes a complicated model with several non-trivial constraints and gives a complicated and non-trivial solution with large approximation ratio.} The literature on duplication is sparse, partly because \hl{it would be quite hard to implement in practice without substantial overhead. It is unclear whether one should be excited about the model's usefulness or for the new important insights into scheduling.}

- Related to the above point, \hl{the paper did not do a good job in explaining the setting of identical machines and what we understand.} The description of past work here is cursory. For instance \hl{the work of [LR02] is cited as providing an algorithm that outputs a schedule with makespan $O((OPT +  \rho) \log \rho/ \log \log \rho)$ for unit sized jobs and delay $\rho$. What about non-uniform sized jobs?} The bound obtained in this paper has an additional log m factor over the identical machine case which is natural since that is the situation even without communication delays and duplication.

- \hl{It is more natural to consider the time indexed formulation. The authors cursorily refer to the one in [KLTY20] as difficult to round but much to my surprise they don't actually say whether the time indexed relaxation is at least as good as two relaxations they write.} Since they spend considerable effort in solving NCP they should indicate whether the time-indexed relaxation would be as strong.

Overall, the paper in its current form did not seem compelling to this reviewer. The authors may wish to revise the paper and address some of the high-level comments.
